Concurrent Composition Theorems for Differential Privacy

We study the concurrent composition properties of interactive differentially private mechanisms, whereby an adversary can arbitrarily interleave its queries to the different mechanisms. We prove that all composition theorems for non-interactive differentially private mechanisms extend to the concurrent composition of interactive differentially private mechanisms, whenever differential privacy is measured using the hypothesis testing framework of $f$-DP, which captures standard $(\eps,\delta)$-DP as a special case. We prove the concurrent composition theorem by showing that every interactive $f$-DP mechanism can be simulated by interactive post-processing of a non-interactive $f$-DP mechanism. In concurrent and independent work, Lyu~\cite{lyu2022composition} proves a similar result to ours for $(\eps,\delta)$-DP, as well as a concurrent composition theorem for R\'enyi DP. We also provide a simple proof of Lyu's concurrent composition theorem for R\'enyi DP. Lyu leaves the general case of $f$-DP as an open problem, which we solve in this paper.

==> Arxiv version/intro.tex <==
%!TEX root = main.tex

\section{Introduction}

\subsection{Differential Privacy}

%The field of {\em differential privacy} \cite{DMNS06} has emerged as the gold standard in private data analysis by providing algorithms with strong worst-case privacy guarantees. 
Differential privacy is a statistical notion of database privacy, which ensures that the output of an algorithm will still have approximately the same distribution if a single data entry were to be changed. Differential privacy can be defined in terms of a general database space $\mathcal{X}$, and a binary {\em neighboring} relation on $\mathcal{X}$, which we think of as capturing whether ``two datasets'' differ on one individual's data.
For example, if databases are real-valued and contain a fixed number $n$ of entries, then $\mathcal{X} = \mathbb{R}^n$, and two datasets $x, x'\in \mathbb{R}^n$ are said to be \emph{neighboring} if they differ in at most one coordinate.

\begin{definition}[Differential Privacy \cite{DMNS06}]\label{def.dp}
	A randomized algorithm $\mathcal{M}: \mathcal{X} \rightarrow \mathcal{R}$ is \emph{$(\epsilon,\delta)$-differentially private} if for every pair of neighboring datasets $x, x'\in \mathcal{X}$, and for every subset of possible outputs $\mathcal{S} \subseteq \mathcal{R}$,
	$$\Pr[\mathcal{M}(x) \in \mathcal{S}] \leq \exp(\epsilon)\cdot \Pr[\mathcal{M}(x') \in \mathcal{S}] + \delta.$$
\end{definition}

Thus, differential privacy requires that for all neighboring datasets $x,x'$, $\mathcal{M}(x)$ and $\mathcal{M}(x') $ are close as probability distributions (as measured by the parameters $\eps$ and $\delta$). A number of variants of differential privacy have been defined based on other ways of measuring closeness, leading to Concentrated differential privacy (CDP) \cite{dwork2016concentrated,bun2016concentrated} and R\'enyi differential privacy (RDP) \cite{mironov2017renyi} and $f$-differential privacy ($f$-DP) \cite{dong2019gaussian}.

%$f$-differential privacy ($f$-DP) is a relaxation of differential privacy based on the hypothesis testing interpretation of differential privacy. Differential privacy attemps to measure the difficulty of distinguishing two neighboring databases based on the ouput of a mechanism. Specifically, an adversary considers the following hypothesis testing problem:
%$$H_0: \text{the dataset is }X \quad \text{versus} \quad H_1: \text{the dataset is }X'.$$
%
%Denote by $P$ and $Q$ the output distributions of $\mathcal{M}$ on the two neighboring datasets, namely $\mathcal{M}(X)$ and $\mathcal{M}(X')$. For a given decision rule $\phi$, the type I error $E_X[\phi]$ is the probaility of rejecting $H_0$ when $H_0$ is true, while type II error $1-E_Y[\phi]$ is the probaility of failing to reject $H_0$ when $H_1$ is true. A trade-off function serves as the optimal boundary of the achievable and unachievable regions of these errors. Neyman-Pearson lemma gives the optimal tests, which can be thought of the most powerful adversaries. 
%
%\begin{definition}[Trade-off Function \cite{dong2019gaussian}]\label{tradeoff.def}
%	For any two probability distributions $P$ and $Q$ on the same space, define the trade-off function $T(P,Q): [0,1]\rightarrow [0,1]$ as
%	\begin{equation}\label{eq.tradeoff}
	%		T(P,Q)(\alpha)=\inf\{\beta_\phi: \alpha_\phi\le \alpha\},
	%	\end{equation}
%	where the infimum is taken over all (measurable) rejection rules $\phi$.
%\end{definition}
%
%
%Proposition \ref{def.tradeoffclass} gives the necessary and sufficient condition for $f$ to be a trade-off function.
%\begin{proposition}[Class of trade-off functions \cite{dong2019gaussian}]\label{def.tradeoffclass}
%	A function $f: [0,1]\rightarrow [0,1]$ is a trade-off function if and only if $f$ is convex, continuous, non-increasing, and $f(x)\le 1-x$ for $x\in [0,1]$.
%\end{proposition}
%
%
%$f$-DP allows the full trade-off between type I and type II errors in the simple hypothesis testing problem to be governed by a trade-off function $f$. A larger trade-off functions implies stronger privacy guarantees.
%
%\begin{definition}[$f$-Differential Privacy \cite{dong2019gaussian}]\label{def.fdp}
%	Let $f$ be a trade-off function. A mechanism $\mathcal{M}$ is $f$-differential private if for every pair of neighboring sets $X,X' \in \mathcal{X}$,
%	$$T(\mathcal{M}(X), \mathcal{M}(X'))\ge f.$$
%\end{definition}
%
%Zero-concentrated differential privacy (zCDP) \cite{dwork2016concentrated,bun2016concentrated} and R\'enyi differential privacy (RDP) \cite{mironov2017renyi} are based on R\'enyi divergence between the output distributions of $\mathcal{M}$ on the two neighboring datasets.
%
%\begin{definition}[R\'enyi differential privacy (RDP) \cite{mironov2017renyi}]
%	A randomized algorithm $\mathcal{M}: \mathcal{X} \rightarrow \mathcal{R}$ is \emph{$(\alpha,\eps)$-RDP} if for every pair of neighboring datasets $x, x'\in \mathcal{X}$,
%	$$D_\alpha(\mathcal{M}(x) || \mathcal{M}(x'))\le \eps.$$
%\end{definition}
%
%\begin{definition}[Zero-Concentrated Differential Privacy (zCDP) \cite{bun2016concentrated}]
%	A randomized algorithm $\mathcal{M}: \mathcal{X} \rightarrow \mathcal{R}$ is \emph{$(\xi,\rho)$-zCDP} if for every pair of neighboring datasets $x, x'\in \mathcal{X}$, and for all $\alpha\in(1,\infty)$,
%	$$D_\alpha(\mathcal{M}(X) || \mathcal{M}(X'))\le \xi +\rho \alpha.$$
%\end{definition}



\subsection{Interactive Differential Privacy}

Definition \ref{def.dp} considers only non-interactive mechanisms $\mathcal{M}$  that release query answers in one shot, but data analysts often interact with a database in an adaptive fashion.  In fact, many useful primitives in differential privacy such as the Sparse Vector Technique \cite{DNRRV09,DNPR10, dwork2014algorithmic}, and the Private Multiplicative Weights \cite{hardt2010multiplicative} allow analysts to ask an adaptive sequence of queries about a dataset. It motivates the study of {\em interactive mechanisms} to capture full-featured privacy-preserving data analytics. Here, we view the mechanism $\mathcal{M}$ as a party in an interactive protocol, interacting with a (possibly adversarial) analyst. 
%The interactive measurement has been used as the basic abstraction in the programming framework in the open-source software project OpenDP \cite{gaboardi2020programming}. In interactive measurement, the mechanism $\mathcal{M}$ is a party interacting with an adversary in an interative protocol.

\begin{definition}[Interactive protocols]\label{def.protocol}
	An  {\em interactive protocol} $(A,B)$ is any pair of functions on tuples of binary strings. The {\em interaction} between $A$ with input $x_A$ and $B$ with input $x_B$ is the following random process (denoted $(A(x_A), B(x_B))$):
	\begin{enumerate}
		\item Uniformly choose random coins $r_A$ and $r_B$ for $A$ and $B$, respectively.
		\item Repeat the following for $i=0,1,\ldots$.\\
		(a) If $i$ is even, let $m_i=A(x_A, m_1, m_3, \ldots, m_{i-1}; r_A)$.\\
		(b) If $i$ is odd, let $m_i=B(x_B, m_0, m_2, \ldots, m_{i-1}; r_B)$.\\
		(c) If $m_{i}=\texttt{halt}$, then exit loop.
	\end{enumerate}
%	We say that $A$ has {\em finite communication} if for every $x_A$ there is a constant $c$, such that for all $r_A, m_1, \ldots, m_{i-1}$, we have 
%	\begin{enumerate}
%		\item If $\max \{i, |m_1|, \ldots, |m_{i-1}|\}>c$, then $A(x_A, m_1, m_3, \ldots, m_{i-1}; r_A)=\texttt{halt}$.
%		\item If $\max \{i, |m_1|, \ldots, |m_{i-1}|\}\le c$, then $ \sum_{j=0}^{i-1} \left| A(x_A, m_1, m_3, \ldots, m_j; r_A)\right| \le c$. 
%	\end{enumerate}
%	Here $|y|$ denotes the bit length of string $y$. $B$ having finite communication is defined symmetrically.
\end{definition}



The view of a party in an interactive protocol captures everything the party ``sees'' during the execution.

\begin{definition}[View of a party in an interactive protocol]
	Let $(A,B)$ be an interactive protocol. Let $r_A$ and $r_B$ be the random coins for $A$ and $B$, respectively. $A$'s view of $(A(x_A;r_A), B(x_B; r_B))$ is the tuple $\View_A ( A(x_A;r_A) \leftarrow B(x_B; r_B) ) = (r_A, x_A, m_1, m_3, \ldots)$ consisting of all the messages received by $A$ in the execution of the protocol together with the private input $x_A$ and random coins $r_A$. $B$'s view of $(A(x_A;r_A), B(x_B; r_B))$ is defined symmetrically.
\end{definition}


%The complexity of an interactive protocol is measured by the number of messages and the communication complexity.
%
%\begin{definition}[Communication complexity]
%	We say that an interactive protocol $(A,B)$ exchanges $m$ messages on input $x$, if for every choice of the random coins for $A$ and $B$, the number of messages computed before the first $\mathrm{accept}/\mathrm{reject}/\mathrm{halt}$ message is at most $m$ (or $m+1$, if the first message $m_1$ of $A$ is always the empty string). 
%	
%	We say that an interactive protocol $(A,B)$ has $A$-to-$B$ (resp., $B$-to-$A$) communication $c$ on input $x$, if for every choice of the random coins for $A$ and $B$, the sum of the lengths of the messages computed by $A$ (resp., $B$) (excluding an $\mathrm{accept}/\mathrm{reject}/\mathrm{halt}$ message) is at most $c$. $(A,B)$ has total communication $c$ on input $x$, if the sum of the lengths of all messages computed (by both $A$ and $B$) is at most $c$ (again, excluding $\mathrm{accept}/\mathrm{reject}/\mathrm{halt}$ messages).
%\end{definition}


In the setting of differentially private mechanisms,  Party $A$ is the mechanism, where the input $x_A$ is the dataset. party $B$ is the adversary that does not have an input $x_B$.  Since we only care about the view of the adversary, we will drop the subscript and denote the view of the adversary as $\View ( B \leftrightarrow  \mathcal{M}(x) )$. With this notation, interactive differential privacy is defined by asking for the views of an adversary on any pair of neighboring datasets $\View ( B \leftrightarrow  \mathcal{M}(x) )$ and $\View ( B \leftrightarrow  \mathcal{M}(x') )$ satisfying the same $(\eps, \delta)$-closeness notion as in non-interactive differential privacy. 

%To provide privacy guarantees, we hope that $View_A\langle A, \mathcal{M}(D_0) \rangle$ and $View_A\langle A, \mathcal{M}(D_1) \rangle$ satisfies a certain closeness notion such as differential privacy or its variants.

\begin{definition}
	A randomized algorithm $\mathcal{M}$ is an  {\em $(\eps,\delta)$-differentially private interactive mechanism} if for every pair of neighboring datasets $X,X'\in\mathcal{X}$, every adversary algorithm $B\in \mathcal{B}$, and every subset of possible views $\mathcal{S} \subseteq \text{Range}(\View )$,  we have 
	
	$$\Pr[ \View ( B \leftrightarrow \mathcal{M}(x) ) \in \mathcal{S}] \leq \exp(\epsilon)\cdot \Pr[ \View (B \leftrightarrow  \mathcal{M}(x') )\in \mathcal{S}] + \delta.$$
	
\end{definition}



\subsection{Concurrent Composition}

A fundamental problem in differential privacy is studying how the privacy degrades under {\em composition} as more computations are performed on the same database. The composition property is particularly useful when we want to ask interactive queries on the same database, and it also allows us to design a complex differentially private algorithm by combining several building blocks. Formally, we define the composition of a sequence of non-interactive $k$ mechanisms $\mathcal{M}_1, \mathcal{M}_2, \ldots, \mathcal{M}_{k}$ as the non-interactive mechanism $\mathcal{M}=\comp (\mathcal{M}_1, \mathcal{M}_2, \ldots, \mathcal{M}_{k}) $ defined as
\begin{equation}
	\mathcal{M}(x):= (\mathcal{M}_1(x), \mathcal{M}_2(x), \ldots, \mathcal{M}_{k}(x)),
\end{equation}
where each mechanism $\mathcal{M}$ is executed using independent random coins. 

%\wz{discuss why previous proof does not work.}


The composition of non-interactive mechanisms has been studied extensively in the literature.
The basic composition theorem \cite{dwork2006our} states that the privacy parameters add up linearly when composing private mechanisms. The advanced composition theorem \cite{dwork2010boosting} provides a tighter bound where the privacy parameter grows sublinearly under $k$-fold adaptive composition. Later, the optimal composition theorem \cite{kairouz2015composition, murtagh2016complexity} gives an exact characterization of the privacy guarantee under $k$-fold composition. The relaxations of differential privacy including zero-concentrated differential privacy (zCDP) \cite{dwork2016concentrated,bun2016concentrated}, R\'enyi differential privacy (RDP) \cite{mironov2017renyi}, and $f$-differential privacy ($f$-DP) \cite{dong2019gaussian} allows for tighter reasoning about composition. 
In the abovementioned work, some of them \cite{dwork2010boosting, murtagh2016complexity} are framed in a way that the adversary can adaptively choose the mechanisms $\mathcal{M}_1, \mathcal{M}_2,\ldots,\mathcal{M}_{k}$, and thus the adaptive composition can be viewed as an interactive mechanism. 

\begin{figure}[H]
	\centering
	\includegraphics[width=.5\textwidth]{protocol.png}
	\caption{Concurrent composition of interactive mechanisms}\label{fig:concomp}
\end{figure}



In many cases, analysts may wish to perform multiple {\em interactive} analyses on the same dataset concurrently, which raises the question of {\em concurrent composition}, first studied for differential privacy in \cite{vadhan2021concurrent}.
%Since the proofs of the sequential composition of non-interactive DP mechanisms can be easily extended to handle the sequential composition of interactive DP mechanisms, the interesting case is that when multiple interactive DP mechanisms run concurrently.  
In this setting (illustrated in Figure \ref{fig:concomp}), an adversary can arbitrarily interleave its queries to several differentially private mechanisms, and those queries might be correlated and depends on the answer received in other mechanisms. As a motivating example, several organizations might set up multiple DP query systems on datasets that may refer to the same set of individuals. Each query system has its own privacy budget $\eps$. Suppose an adversary can concurrently access those systems, and a query sent to one system might depends on all the previous messages that received from other systems. For example, when we run two Sparse Vector mechanisms $\mathcal{M}_1$ and $\mathcal{M}_2$ concurrently, the queries for $\mathcal{M}_1$ depends on previous answers from $\mathcal{M}_2$, and vice-versa, but we only know the overall privacy guarantees for $\mathcal{M}_1$ and $\mathcal{M}_2$ when they are executed independently. 
%Directly using sequential composition technique is not applicable for analyzing the concurrent composition. %\new{The previous proof technique decomposes the overall output probability using the chain rule of conditional probability: $\Pr( (\mathcal{M}_1, \ldots, \mathcal{M}_k)= (a_1, \ldots, a_k)  )=\Pr(\mathcal{M}_1=a_1)\Pr(\mathcal{M}_2=a_2|\mathcal{M}_1=a_1)\ldots\Pr(\mathcal{M}_k=a_k| \mathcal{M}_1, \ldots, \mathcal{M}_{k-1}= (a_1, \ldots, a_{k-1}))$. However, we can no longer decompose the probability in this way for concurrent composition,  because the output of $\mathcal{M}_1, \ldots, \mathcal{M}_{k-1}$ also depends on the output of $\mathcal{M}_k$.  }
%\new{In previous proofs, the privacy loss from interacting with different mechanisms is independent of each other, which is because the adversary already knows all the messages from previous mechanisms, and the adversary interacts with the mechanisms with a fixed strategy. Because of this independence, we can simply sum up the privacy losses from different mechanisms. However, for concurrent composition, the privacy losses from interacting with different mechanisms are no longer independent, since the strategy of the adversary may change, depending on the messages from other mechanisms.}
If the executions were {\em sequential}, meaning that the adversary completes its interaction with $\mathcal{M}_1$ before issuing any queries to $\mathcal{M}_2$, then we can hardwire the answers from   $\mathcal{M}_1$ into the adversary's strategy. When attacking $\mathcal{M}_2$, the privacy loss for $\mathcal{M}_2$ will be bounded as usual. But when the queries are interleaved, it is no longer clear how to define a fixed adversary strategy against either of the mechanisms $\mathcal{M}_1$ or $\mathcal{M}_2$.
It is not clear if the adversary can run any concurrent attack to break the privacy guarantees, and therefore, we wish to provide a provable guarantee to account for the total privacy loss in such systems. Formally, the concurrent composition of interactive mechanisms is defined as follows.

\begin{definition}[Concurrent composition of interactive mechanisms\cite{vadhan2021concurrent}]
	Let $\mathcal{M}_1,\ldots, \mathcal{M}_{k}$ be interactive mechanisms. $\mathcal{M}=ConComp(\mathcal{M}_1,\ldots, \mathcal{M}_{k})$ is the concurrent composition of mechanisms $\mathcal{M}_1,\ldots, \mathcal{M}_{k}$ defined as follows:
	\begin{enumerate}
		\item Random sample $r=(r_1,\ldots,r_{k})$ where $r_j$ are random coin tosses for $\mathcal{M}_j$.
		\item Inputs for $\mathcal{M}$ consists of $x=(x_1,\ldots,x_{k})$ where $x_j$ is a private dataset for $\mathcal{M}_j$. 
		\item $\mathcal{M}(x,m_0,\ldots,m_{i-1};r)$ is defined as follows:
		\begin{enumerate}
			\item Parse $m_{i-1}$ as $(j,q)$ where $j=1, \ldots, k$ and $q$ is a query to $\mathcal{M}_j$. If $m_{i-1}$ cannot be parsed correctly, output $\texttt{halt}$.
			\item Extract history $(m_0^j,\ldots,m_{t-1}^j)$ from $(m_0,\ldots,m_{i-1})$ where $m_i^j$ are all of the queries to mechanism $\mathcal{M}_j$. 
			\item Output $\mathcal{M}_j(x_j, m_0^j,\ldots,m_{t-1}^j; r_j)$.
		\end{enumerate}
	\end{enumerate}
For an adversary $B$, we will use the notation $\View(B\leftrightarrow (\mathcal{M}_1,\ldots, \mathcal{M}_{k}))$ as shorthand for $\View(B\leftrightarrow \concomp(\mathcal{M}_1,\ldots, \mathcal{M}_{k}))$
\end{definition}


%This desideratum has motivated the study of {\em concurrent composition} of interactive differentially private mechanisms \cite{vadhan2021concurrent}.


Vadhan and Wang \cite{vadhan2021concurrent} showed that the advanced and optimal composition theorems extend to the concurrent composition of interactive pure DP mechanisms.

\begin{theorem}[\cite{vadhan2021concurrent}]\label{thm.puredpconcomp}
	Suppose that for all non-interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ such that $\mathcal{M}_i$ is $(\eps_i, \delta_i)$-differentially private for $\delta_1=\delta_2=\ldots=\delta_k=0$, their composition $\comp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ is $(\eps, \delta)$-differentially private. Then for all interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ such that $\mathcal{M}_i$ is $(\eps_i, \delta_i)$-differentially private for $\delta_1=\delta_2=\ldots=\delta_k=0$, 
	the concurrent composition $\concomp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ of interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ is $(\eps, \delta)$-differentially private.
\end{theorem}



They prove this by reducing the analysis of interactive pure DP mechanism to that of analyzing the Randomized Response mechanism \cite{warner1965randomized,DMNS06}:


\begin{theorem}[\cite{vadhan2021concurrent}]\label{thm.puredptoRR}
	Suppose that $\mathcal{M}$ is an interactive $(\eps, 0)$-differentially private mechanism. Then for every pair of neighboring datasets $x, x'$, there exists an interactive post-processing function $\mathcal{P}$  such that for every adversary $B \in \mathcal{B}$, we have 
	\begin{align}
		\View(B \leftrightarrow  \mathcal{M}(x))\equiv \View(B \leftrightarrow  \mathcal{P}(RR_\eps(0)))
		&&
		\View(B \leftrightarrow  \mathcal{M}(x'))\equiv \View(B \leftrightarrow \mathcal{P}(RR_\eps(1))).
	\end{align}
\end{theorem}

Here $\mathcal{P}$ is an interactive post-processing function that depends on $\mathcal{M}$ and a fixed pair of neighboring datasets $x, x'$. It receives a single bit as an output of $RR_\eps(0)$ or $RR_\eps(1)$, and then interacts with the adversary $A$.
%Following this result, to analyze $\concomp (\mathcal{M}_1, \ldots, \mathcal{M}_{k})$, we only need to analyze $\comp (RR_{\eps_1}, \ldots, RR_{\eps_k})$, which is the composition of non-interactive mechanisms.

Note that Theorem \ref{thm.puredpconcomp} and Theorem \ref{thm.puredptoRR} do not apply to the case where the composed mechanisms $\mathcal{M}_i$ are $(\eps_i,\delta_i)$-DP for $\delta_i>0$. In this case, \cite{vadhan2021concurrent} only show a bound that is similar to the ``group privacy'' property of $(\eps,\delta)$-DP. In particular, if $\eps_1=\eps_2=\ldots=\eps_k=\eps$ and $\delta_1=\delta_2=\ldots=\delta_k=\delta$, they show 
that the concurrent composition $\concomp(\mathcal{M}_1, \mathcal{M}_2, \ldots, \mathcal{M}_{k})$ is $(k\eps, \frac{\exp(k\eps)-1}{\exp(\eps)-1}\delta)$-differentially private.
This is suboptimal even compared to basic composition.
It left as an open problem that if any composition theorems for non-interactive mechanisms can extend to all variants of DP interactive mechanisms.
%\begin{theorem}[\cite{vadhan2021concurrent}]
%For any $(\eps,\delta)$-differentially private interacitve mechanism $\mathcal{M}_1, \mathcal{M}_2, \ldots, \mathcal{M}_{k}$, their $\concomp(\mathcal{M}_1, \mathcal{M}_2, \ldots, \mathcal{M}_{k})$ is $(k\eps, \frac{\exp(k\eps)-1}{\exp(\eps)-1}\delta)$-differentially private.
%\end{theorem}

\paragraph{Open Question.} Does Theorem \ref{thm.puredpconcomp} extend to other variants of DP (such as $(\eps_i,\delta_i)$-DP with $\delta_i>0$, R\'enyi DP, $f$-DP)?

%For all variants of DP ($(\eps,\delta)$-DP, $f$-DP, RDP and zCDP), does the follow equation hold?
%\begin{equation*}
%	\concomp(\mathcal{M}_1, \mathcal{M}_2, \ldots, \mathcal{M}_{k})  = \comp (\mathcal{M}_1, \mathcal{M}_2, \ldots, \mathcal{M}_{k})
%\end{equation*}






\subsection{Our Results on Concurrent Composition}

In this paper, we close this gap and show that any composition theorems of non-interactive mechanisms also extend to the concurrent composition of interactive DP mechanisms for approximate DP. In particular, we show that Theorem \ref{thm.puredpconcomp} extends to the case that $\delta_i>0$:
%including $(\eps,\delta)$-DP (Theorem \ref{thm.concomp}), $f$-DP (Theorem \ref{thm.fdp}), RDP/zCDP (Theorem \ref{thm.rdp}). With more platforms of differential privacy that allow for full interactivity with the private being deployed in practice, our work can provide guidance on accounting for the total privacy loss on concurrent private data analyses. 



\begin{theorem}[Concurrent composition for $(\eps, \delta)$-DP interactive mechanisms]\label{thm.concomp}
	Suppose that for all non-interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ such that $\mathcal{M}_i$ is $(\eps_i, \delta_i)$-differentially private for $i=1,2 \ldots, k$, their composition $\comp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ is $(\eps, \delta)$-differentially private. Then for all interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ with finite communication such that $\mathcal{M}_i$ is $(\eps_i, \delta_i)$-differentially private for $i=1,2 \ldots, k$, 
	the concurrent composition $\concomp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ of interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ is $(\eps, \delta)$-differentially private.
\end{theorem}

We also handle general $f$-DP as defined and discussed in the section below.

\begin{theorem}[Concurrent composition for $f$-DP interactive mechanisms]\label{thm.fdp} 
	Suppose that for all non-interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ such that $\mathcal{M}_i$ is $f_i$-DP for $i=1,2 \ldots, k$, their composition $\comp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ is $f$-DP. Then for all interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ such that $\mathcal{M}_i$ is $f_i$-DP for $i=1,2 \ldots, k$, 
	the concurrent composition $\concomp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ of interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ is $f$-DP.
\end{theorem}
%\sv{expanded thm statement}

%\begin{theorem}[Concurrent compostion for RDP interactive mechanisms]\label{thm.rdp}
%	%	Suppose that for all non-interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ such that $\mathcal{M}_i$ is $(\alpha,\eps_i)$-RDP for $i=1,2 \ldots, k$, their composition $\comp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ is $(\alpha,\eps)$-RDP. Then for all interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ such that $\mathcal{M}_i$ is $(\alpha,\eps_i)$-RDP for $i=1,2 \ldots, k$, 
%	%	the concurrent composition $\concomp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ of interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ is $(\alpha,\eps)$-RDP.
%	The analogue of Theorem \ref{thm.concomp} holds for R\'enyi DP of any fixed order.
%\end{theorem}

%When $\alpha$ is fixed, then the optimal non-interactive RDP composition is $(\alpha, \sum_i \eps_i)$.

Theorem \ref{thm.concomp} follows directly from Theorem \ref{thm.fdp} because $f$-DP defined below captures $(\eps, \delta)$-DP as a special case 
\cite{wasserman2010statistical, dong2019gaussian}. Interestingly, the generalization to $f$-DP is important for our proof, even if we only want to prove Theorem \ref{thm.concomp}.
 We explain the detailed proof technique in the section below. 

In summary, our results show that there is no extra privacy loss due to the concurrent access to multiple interactive mechanisms. We can now safely run multiple interactive differentially private algorithms in parallel, while allowing communication with all them during their executions.

 
%In fact, we prove Theorem \ref{thm.reduction} under the more general relaxation $f$-DP, which captures $(\eps, \delta)$-DP as a special case 
%\cite{wasserman2010statistical, dong2019gaussian}, and thus, we claim that Theorem \ref{thm.reduction} holds for $(\eps, \delta)$-DP. We will provide explanation of why we approach it by first considering $f$-DP in the proof sketch.
%To prove Theorem \ref{thm.fdp}, our key insight is to show that any interactive $f$-DP mechanisms can be simulated by interactive post-processing of a non-interactive $f$-mechanism. This is a generalization of the result in \cite{vadhan2021concurrent} that any interactive $\eps$-DP algorithm can be viewed as an interactive post-processing of $\eps$-randomized response. 
%This is a generalization of the results in \cite{kairouz2015composition} that any $(\eps,\delta)$-DP algorithm can be viewed as randomized post-processing of $(\eps, \delta)$-randomized response. 
%Our proof is based on the hypothesis testing interpretation of differential privacy. Specifically, we take the view of differential privacy as characterizing the type I and type II errors in a binary hypothesis testing problem which is distinguishing two neighboring databases based on the output of a mechanism. Since $f$-DP allows the full trade-off between type I and type II errors in the simple hypothesis testing problem, we show such property of reduction to non-interactive mechanisms holds for $f$-DP, and thus, any composition theorems of non-interactive mechanisms also extend to the concurrent composition of interactive $f$-DP mechanisms.

%To prove Theorem \ref{thm.rdp}, we show a decomposition for R\'enyi divergence between the views of an adversary against the concurrent composition of several interative mechanisms, and thus bound the overall divergence by the divergence for each individual mechanism.  \todo{fill out this later}


%We explain the detailed proof techniques for Theorem \ref{thm.fdp} and Theorem \ref{thm.rdp} in Section \ref{sec.introfdp} and Section \ref{sec.intrordp}, respectively. 


\subsection{$f$-DP and Interactive vs. Noninteractive Hypothesis Testing}\label{sec.introfdp}
%\sv{renamed section}

$f$-differential privacy ($f$-DP) \cite{dong2019gaussian} is a generalization of $(\eps,\delta)$-differential privacy based on the hypothesis testing interpretation of differential privacy. Differential privacy attemps to measure the difficulty of distinguishing two neighboring datasets based on the ouput of a mechanism. Specifically, an adversary considers the following hypothesis testing problem:
$$H_0: \text{the dataset is }x \quad \text{versus} \quad H_1: \text{the dataset is }x'.$$

Denote by $Y$ and $Y'$ the output distributions of $\mathcal{M}$ on the two neighboring datasets, namely $\mathcal{M}(x)$ and $\mathcal{M}(x')$. For a given rejection rule $\phi$, the type I error $\alpha_\phi=\mathrm{E}[\phi(Y)]$ is the probability of rejecting $H_0$ when $H_0$ is true, while the type II error $\beta_\phi=1-\mathrm{E}[\phi(Y')]$ is the probability of failing to reject $H_0$ when $H_1$ is true. A trade-off function serves as the optimal boundary of the achievable and unachievable regions of these errors. 
%Neyman-Pearson lemma gives the optimal tests, which can be thought of the most powerful adversaries. 

\begin{definition}[Trade-off function \cite{dong2019gaussian}]\label{tradeoff.def}
	For any two probability distributions $Y$ and $Y'$ on the same space, define the {\em trade-off function} $T(Y,Y'): [0,1]\rightarrow [0,1]$ as
	\begin{equation}\label{eq.tradeoff}
		T(Y,Y')(\alpha)=\inf\{\beta_\phi: \alpha_\phi\le \alpha\},
	\end{equation}
	where the infimum is taken over all (measurable) rejection rules $\phi$.
\end{definition}


Proposition \ref{def.tradeoffclass} gives the necessary and sufficient condition for $f$ to be a trade-off function.
\begin{proposition}[Class of trade-off functions \cite{dong2019gaussian}]\label{def.tradeoffclass}
	A function $f: [0,1]\rightarrow [0,1]$ is a trade-off function if and only if $f$ is convex, continuous, non-increasing, and $f(x)\le 1-x$ for $x\in [0,1]$.
\end{proposition}


$f$-DP allows the full trade-off between type I and type II errors in the simple hypothesis testing problem to be governed by a trade-off function $f$. A larger trade-off functions implies stronger privacy guarantees.

\begin{definition}[$f$-differential privacy \cite{dong2019gaussian}]\label{def.fdp}
	Let $f$ be a trade-off function. A mechanism $\mathcal{M}: \mathcal{X} \rightarrow \mathcal{R}$  is {\em $f$-differentially private} if for every pair of neighboring datasets $x,x' \in \mathcal{X}$, we have
	$$T(\mathcal{M}(x), \mathcal{M}(x'))\ge f.$$
\end{definition}

$(\eps, \delta)$-DP is a special case of $f$-DP, taking $f=f_{\eps,\delta}$, where $f_{\eps,\delta}=\max\{0, 1-\delta-\exp(\eps)\alpha, \exp(-\eps)(1-\delta-\alpha)\}$ \cite{wasserman2010statistical, dong2019gaussian}. 

To prove Theorem \ref{thm.fdp} (and hence Theorem \ref{thm.concomp}), we prove the following analogue of Theorem \ref{thm.puredptoRR}, showing that every interactive $f$-DP mechanism can be simulated by an interactive post-processing of a non-interactive mechanism. 


\begin{theorem}\label{thm.reduction}
	For every trade-off function $f$, every interactive $f$-DP mechanism $\mathcal{M}$ with finite communication, and every pair of neighboring datasets $x, x'$, there exists a non-interactive $f$-DP mechanism $\mathcal{N}$ and an randomized interactive post-processing mechanism $\mathcal{P}$ such that for every adversary $B \in \mathcal{B}$, we have 
	\begin{align}
		\View(B \leftrightarrow  \mathcal{M}(x))\equiv \View(B \leftrightarrow  \mathcal{P}(\mathcal{N}(x)))
		&&
		\View(B \leftrightarrow  \mathcal{M}(x'))\equiv \View(B \leftrightarrow  \mathcal{P}(\mathcal{N}(x'))).
	\end{align}
\end{theorem}
%\sv{this theorem should also say ``every interactive $f$-DP mechanism $\mathcal{M}$ with finite communication''}
Similarly to Theorem \ref{thm.puredptoRR}, in the case of $(\eps,\delta)$-DP, one can take the non-interactive mechanism $\mathcal{N}$ as the $(\eps,\delta)$-Randomized Response mechanism of \cite{kairouz2015composition}.
Indeed, \cite{kairouz2015composition} shows that every non-interactive $(\eps,\delta)$-DP mechanism can be simulated as a post-processing of $(\eps,\delta)$-Randomized Response.
%\cite{lyu2022composition} extends this result to every interactive $(\eps,\delta)$-DP mechanism. 

Theorem \ref{thm.fdp} follows from Theorem \ref{thm.reduction} in the same way as Theorem \ref{thm.puredpconcomp} follows from Theorem \ref{thm.puredptoRR}. Indeed, Theorem \ref{thm.fdp} implies that
to analyze the concurrent composition of interactive mechanisms $\mathcal{M}_i$, it suffices to consider the composition of the non-interactive mechanisms $\mathcal{N}_i$. As a result, composition theorems for non-interactive mechanisms extend to the concurrent composition of interactive $f$-DP  mechanisms. 

\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}

%\sv{new paragraph below}
Theorem \ref{thm.reduction} is an interesting statement about statistical hypothesis testing even without the application to differential privacy.  Normally, hypothesis testing is presented as the task of distinguishing between two distributions or sets of distributions.  This is a noninteractive task: a sample from the distribution is generated and given to the hypothesis tester, which then tries to decide whether the distribution is in $H_0$ or $H_1$.  However, suppose instead we consider the task of distinguishing between two interactive mechanisms $\cM_0$ and $\cM_1$, each of which responds to queries in a randomized and stateful manner. Since the mechanisms are stateful, the hypothesis tester may never learn everything there is to know about the mechanism; in particular it cannot find out how the mechanism would have answered if different queries had been asked in the past.  This is in contrast to ordinary hypothesis testing, where the full sample from the distribution is given to the hypothesis tester.  Nevertheless, by viewing $\cM_0$ as $\cM(x)$ and $\cM_1$ as $\cM(x')$, Theorem~\ref{thm.reduction} implies that the two interactive mechanisms $\cM_0$ and $\cM_1$ can be simulated perfectly by noninteractive random variables $\cN_0=\cN(x)$ and $\cN_1=\cN(x')$ such that even if we give $\cN_0$ or $\cN_1$ to a hypothesis tester in its entirety (thereby revealing how $\cM_0$ or $\cM_1$ would answer {\em all} questions), it cannot distinguish them any better than it could distinguish $\cM_0$ and $\cM_1$.  The trick, of course, is that the simulation is ``perfect'' only when executing a single interaction with $\cM_0$ or $\cM_1$ (with no rewinding to explore multiple paths in the interaction tree). 


\iffalse
Since $f$-DP is based on the hypothesis testing interpretation of differential privacy and it allows  the full trade-off between type I and type II errors in the simple hypothesis testing problem. Theorem \ref{thm.reduction} implies a nice property of reducing interactive hypothesis testing to non-interactive hypothesis testing. 


\wz{check this paragraph and the theorem}

In the interactive hypotheis testing setting, multiple correlated sources interact with each other to decide between two hypotheses $H_0$ and$H_1$ on the joint distribution of the sources. Suppose we have two interactive boxes $\mathcal{M}, \mathcal{M}'$, which can be viewed as data processing procedures under $H_0$ and $H_1$. Then there exists two non-interactive random variables $\mathcal{N},\mathcal{N}'$ with exactly the same trade-off function, such that $\mathcal{M}, \mathcal{M}'$ can be simulated by interactive post-processing of the non-interactive random variables $\mathcal{N},\mathcal{N}'$. 

\begin{theorem}\label{thm.ht}
	For every trade-off function $f$, and every pair of interactive data processing procedures $\mathcal{M}, \mathcal{M}'$ such that the trade-off function $T(\mathcal{M}, \mathcal{M}')\ge f$. There exists a pair of non-interactive random variables $\mathcal{N},\mathcal{N}'$ and an interactive post-processing mechanism $\mathrm{Proc}$  such that $T(\mathcal{N}, \mathcal{N}')\ge f$, and 
	\begin{align*}
		\mathcal{M} \equiv \mathrm{Proc}(\mathcal{N})
		&&
		\mathcal{M}'\equiv \mathrm{Proc}(\mathcal{N}').
	\end{align*}
\end{theorem}
\fi

%To see the implication for privacy, we consider the hypothesis testing interpretation of differential privacy where we characterize the type I and type II errors in a binary hypothesis testing problem distinguishing two neighboring databases based on the output of a mechanism. 
%Since $f$-DP allows the full trade-off between type I and type II errors in the simple hypothesis testing problem, such a property of reduction implies that any interactive $f$-DP mechanisms can be simulated by post-processing of non-interacitve $f$-DP mechanisms.


The proof of Theorem \ref{thm.reduction} relies on the following two lemmas. 

%\begin{lemma}[Coupling Property of $f$-DP]\label{lemma.coupling}
%	Let $f$ be a trade-off function, and suppose we have random variables $X_0$, $X_1$  and $X'_0$, $X'_1$ such that 
%	\begin{equation*}
	%		T(X_0,X'_0) \ge f \quad \text{and} \quad T(X_1,X'_1)\ge f,
	%	\end{equation*}
%	for any trade-off function $f$.
%	Then there exists random variables $Y=(Y_0, Y_1)$ and $Y'=(Y'_0, Y'_1)$, such that  $Y_q \equiv X_q$ and $Y'_q \equiv X'_q$   hold for any $q\in\{0,1\}$, and we have
%	\begin{equation*}
	%		T((Y_0,Y_1)||(Y'_0,Y'_1))\ge f.
	%	\end{equation*}
%\end{lemma}

\begin{lemma}[Coupling property of $f$-DP]\label{lemma.coupling}
	Let $f$ be a trade-off function, and suppose we have random variables $X$, $Y$  and $X'$, $Y'$ such that 
	\begin{equation*}
	T(X,X') \ge f \quad \text{and} \quad T(Y,Y')\ge f.
\end{equation*}
Then there exists couplings $(X,Y)$ and $(X',Y')$ such that
\begin{equation*}
	T((X,Y)||(X',Y'))\ge f.
\end{equation*}
\end{lemma}



A coupling of random variables $X$ and $Y$ is any random vector $(\tilde{X}, \tilde{Y})$ such that the marginal distributions are identically distributed to $X$ and $Y$ respectively, i.e., $\tilde{X} \equiv X$ and $\tilde{Y} \equiv Y$. Subject to this constraint on the marginal, $\tilde{X}$ and $\tilde{Y}$ can be arbitrarily correlated. Allowing correlations is critical to Lemma \ref{lemma.coupling}.
For example, for the case of $(\eps,\delta)$-DP, if we keep $X, Y$ and $X', Y'$ independent, then we would just get the ``group privacy'' like bound. 

%We use a coupling is to relate $X_0$ and $X_1$ ($X'_0$ and $X'_1$) in a particularly desirable way so that the trade-off function is still characterized by the same $f$.


\begin{lemma}[Chain rule of $f$-DP]\label{lemma.chain}
	For every pair of random variables $X, X'$ with finite support, there exists a function $\mathrm{ChainRule}_{X,X'}$ such that for every random variable $Y$ jointly distributed with $X$, and every random variable $Y'$ jointly distributed with $X'$, we have 
	\begin{equation*}
		T((X,Y), (X',Y'))=\mathrm{ChainRule}_{X,X'}((T(Y|X=x, Y'|X'=x)))_{x\in \supp(X)\cap \supp(X') }).
	\end{equation*}
	Moreover, $\mathrm{ChainRule}$ is a function that is ``continuous in each variable'' on the partially ordered set of trade-off functions (see Section \ref{sec.dDP} for formal definition).
\end{lemma}




Lemma \ref{lemma.chain} says that the trade-off function between $(X, Y)$ and $(X',Y')$ can be determined by a collection of trade-off functions between $Y$ and $Y'$ conditioned on $X=X'=x$ for every $x\in \supp(X)\cap \supp(X')$ through a $\mathrm{ChainRule}$ function.
The terminology ``chain rule'' is by analogy with the standard chain rule for KL divergence, which says

\begin{equation}\label{chain.KL}
\mathrm{KL}((X,Y)||(X',Y'))=\mathrm{KL}(X||X')+\mathrm{E}_{x\sim X}\mathrm{KL}(Y|X=x|| Y'|X'=x).
\end{equation}
So fixing $X$ and $X'$, we can calculate the KL divergence for arbitrary $Y$ and $Y'$ as a function of the KL divergences $\mathrm{KL}(Y|X=x|| Y'|X'=x)$.
 $(\eps,\delta)$-DP does not admit the chain rule property, because no pairs of $(\eps, \delta)$ can exactly capture the ``closeness'' of $(X,Y)$ and $(X',Y')$ given a collection of $\{\eps_j, \delta_j\}_j$ that characterize the ``closeness'' of $Y|X=x$ and $Y'|X'=x'$. Working with the general $f$-DP allows us to capture a complete characterization of ``privacy''.


To prove Theorem \ref{thm.reduction} using Lemmas \ref{lemma.coupling} and \ref{lemma.chain}, our strategy is to apply induction on  the number of messages exchanged (which we can do since $\mathcal{M}$ has finite communication by assumptions). To reduce $k$ rounds of interactions to $k-1$ rounds, we consider the subsequent interaction conditioned on the first message. Depending on whether the first message sent from the mechanism $\mathcal{M}$ or the adversary $B$, we consider the following two cases. 

\textbf{Case 1.} The adversary $B$ sends the first query $q_1$ to the mechanism $\mathcal{M}$. Fix a pair of neighboring datasets $x, x'$. Fixing $q_1$, we denote the subsequent interactive mechanism by $\mathcal{M}_{q_1}$. By induction, $\mathcal{M}_{q_1}$ can be simulated by a post-processing of a non-interactive $f$-DP mechanism $\mathcal{N}_{q_1}$. 
Then we obtain $\mathcal{N}(x)$ and $\mathcal{N}(x')$ by coupling the pairs $\mathcal{N}_{q_1}(x)$ and $\mathcal{N}_{q_1}(x')$ on all the values of $q_1$, which is finite by our assumption of finite communication. We note that the coupling lemma  \ref{lemma.coupling} extends to finite number of random variables $ Y_1, \ldots, Y_k$ and $Y'_1, \ldots, Y'_k$ by induction on $k$. Following the coupling lemma, we have $T(\mathcal{N}(x), \mathcal{N}(x') )\ge f$.
We can combine the interactive post-processing mechanisms $\mathcal{P}_{q_1}$ for all $q_1$ to obtain the interactive post-processing $\mathcal{P}$ that simulates $\mathcal{M}(x)$ and $\mathcal{M}(x')$ from $\mathcal{N}(x)$ and $\mathcal{N}(x')$. Thus, we have Theorem \ref{thm.reduction} holds for $k$ rounds of interactions. 

\begin{figure}[H]
	\centering
	\includegraphics[width=0.8\textwidth]{coupling.png}
	\caption{Case 1: The adversary $B$ sends the first query $q_1$.}\label{fig:coupling}
\end{figure}


%Then following Lemma \ref{lemma.coupling}, there exists a pair of couplings $Y, Y'$ of all possible subsequent interactions $\{\mathcal{N}_{q_1}\}$ on $x,x'$ such that $T(Y, Y')\ge f$. Since $Y, Y'$ are obtained by post-processing of the non-interactive mechanisms $\{\mathcal{N}_{q_1}\}$, we have Theorem \ref{thm.reduction} holds for $k$ rounds of interactions. 

\textbf{Case 2.} The mechanism $\mathcal{M}$ sends the first message $a_1$ to the adversary $B$. Fix a pair of neighboring datasets $x, x'$. We denote the mechanism conditioned on every $a_1$ by $\mathcal{M}_{a_1}$, and let $f_{a_1}$ be the trade-off function of  $\mathcal{M}_{a_1}$ (maximized over all adversaries). We denote the random variable of the first message as $A_1, A'_1$ on datasets $x,x'$, respectively. 
%Following lemma \ref{lemma.chain},  the trade-off function $T((A_1, M_{A_1}(x)), (A'_1, M_{A'_1}(x')))$ can be determined by the ChainRule function of the set of all possible trade-off functions conditioned on $a_1\in \supp(A_1)\cap \supp(A'_1)$. 
By induction, $\mathcal{M}_{a_1}$ can be simulated by a post-processing of a non-interactive $ f_{a_1}$-DP mechanism $\mathcal{N}_{a_1}$.
% and therefore, we have $$T(\mathcal{N}_{a_1}(x), \mathcal{N}_{a_1}(x')) \ge T(\mathcal{M}_{a_1}(x), \mathcal{M}_{a_1}(x')) \ge f_{a_1}.$$ We apply the ChainRule function again on $T((A_1, N_{A_1}(x)), (A'_1, N_{A'_1}(x')))$, using the fact that $\mathrm{ChainRule}$ is a continuous monotone function, we deduce $$T((A_1, N_{A_1}(x)), (A'_1, N_{A'_1}(x')))= T((A_1, M_{A_1}(x)), (A'_1, M_{A'_1}(x')))\ge f.$$
%Moreover, we can view $(A_1, M_{A_1})$ as a post-processing of $(A_1, N_{A_1})$, which is non-interactive. 
Thus, $\mathcal{M}$ can be simulated by a post-processing of the non-interactive mechanism $\mathcal{N}$ where $\mathcal{N}(x) \equiv (A_1, \mathcal{N}_{A_1}(x))$ and $\mathcal{N}(x') \equiv (A'_1, \mathcal{N}_{A'_1}(x'))$. We use the chain rule to argue that $T( \mathcal{N}(x), \mathcal{N}(x')  )\ge  \mathrm{ChainRule}_{A_1,A'_1}\left(  (f_{a_1})_{a_1\in \supp(A_1)\cap\supp(A'_1)} \right) =f$.
We conclude that Theorem \ref{thm.reduction} holds for $k$ rounds of interactions. 

\begin{figure}[H]
\centering
\includegraphics[width=0.8\textwidth]{chainrule.png}
\caption{Case 2: The mechanism $\mathcal{M}$ sends the first message $a_1$. }\label{fig:chain}
\end{figure}



%In fact, we prove Theorem \ref{thm.reduction} under the more general relaxation $f$-DP, which captures $(\eps, \delta)$-DP as a special case 
%\cite{wasserman2010statistical, dong2019gaussian}, and thus, we claim that Theorem \ref{thm.reduction} holds for $(\eps, \delta)$-DP. We will provide explanation of why we approach it by first considering $f$-DP in the proof sketch.

%	\begin{proof}[Proof Sketch for Theorem \ref{thm.reduction}]
	%		To prove Theorem \ref{thm.reduction}, our strategy is to apply the induction argument by the number of rounds of interactions. Fix a pair of neighboring datasets $x, x'$. We consider two cases depending on whether the first message sent from the mechanism $\mathcal{M}$ or the adversary $A$. In the first case, the adversary $A$ sends the first query $q_1$ to the mechanism $\mathcal{M}$. 
	%		Conditioned on $q_1$, we denote the subsequent interactive mechanism $\mathcal{M}_{q_1}$. For any $q_1$, $View ( A, \mathcal{M}_{q_1})$ consists of $m-1$ messages, and $\mathcal{M}_{q_1}$ satisfies $(\eps, \delta)$-DP. By induction, there exists an interactive post-processing $T_{q_1}$ and a non-interactive $(\eps, \delta)$-DP mechanism $\mathcal{N}_{q_1}$ such that $\mathcal{M}_{q_1}$ can be simulated by $T_{q_1}(\mathcal{N}_{q_1})$.  By Theorem 2.5 in \cite{kairouz2015composition}  (see also the Blackwell theorem  \cite{blackwell1953equivalent}), there exists a stochastic post-processing $S_{q_1}$ that takes in $RR_{\eps, \delta}(b)$ that ouput has the same marginal distribution as $\mathcal{N}_{q_1}$ conditioned on the dataset. Let $T=T_{q_1}\cdot S_{q_1}$, then the mechanism $\mathcal{M}$  can be simulated by $T$ of $RR_{\eps, \delta}(b)$. We note that $f$-DP has the same ``coupling'' property due to the Blackwell theorem \cite{dong2019gaussian}. 
	%		
	%		In the second case, the mechanism $\mathcal{M}$ sends the first answer $a$ to the adversary $A$. We will need another property called the ``Chain Rule' for a given divergence $D$:  for every pair of random variables $(X, X')$ on the same domain, there exists a continuous function $ChainRule_{X,X'}$ such that for every pair of random variables $Y, Y'$ where $Y$ is jointly distributed with $X$ and $Y'$ is jointly distributed with $X'$, we have $D((X,Y),(X',Y')) = ChainRule_{X,X'}((D(Y|X=x,Y'|X'=x)_{x \in supp(X) \cap supp(X')}).$ Intuitively, the Chain Rule says that the divergence of the joint distribution $D((X,Y),(X',Y'))$ can be exactly captured by a set of divergence of the conditional distributions $(D(Y|X=x,Y'|X'=x)$. Unfortunately, $(\eps,\delta)$-DP does not enjoy the Chain Rule property, where the divergence is the $\delta$-approximate max-divergence. Nevertheless, $f$-DP satisfies the Chain Rule property because the trade-off function, which is the divergence $D$ here, gives optimal boundary of type I and type II errors in the simple hypothesis testing problem. The argument for $f$-DP mechanisms in the second case is as follows.
	%		For any $a$ from the joint of the output supports given $x, x'$,  suppose the subsequent interactive mechanism $\mathcal{M}_a$ is $f_a$-DP, then by induction, $\mathcal{M}_a$ can be reduced to a pair of random variables $Y_a, Y'_a$ that characterize the output of non-interactive $f_a$-DP mechanism $\mathcal{N}_a$ given datasets $x, x'$. Let $X, X'$ be the random variable of the first answer $a$ given dataset $x, x'$, respectively. Then, the interactive mechanism $\mathcal{M}$ can be reduced to the pair of random variable $(X, Y_X), (X, Y'_X)$, and it satisfies $f$-DP followed by the Chain Rule.
	%		
	%		
	%	\end{proof}






%	\begin{corollary}[Concurrent Compostion]\label{thm.concomp}
	%		Suppose that for all non-interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ such that $\mathcal{M}_i$ is $(\eps_i, \delta_i)$-differentially private for $i=1,2 \ldots, k$, their composition $\comp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ is $(\eps, \delta)$-differentially private, then the concurrent composition $\concomp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ of interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ is also $(\eps, \delta)$-differentially private.
	%	\end{corollary}
%	



%In Section \ref{sec.dDP}, we consider the concurrent composition using a bigger abstraction of differential privacy. Specifically, the difficulty of distinguishing two neighboring datasets is measured by a generalized distance between the distributions of an adversary's views. We define privacy in terms of the generalized distance under certain conditions. Therefore, our results can be extended to a pair of random variables that are close with respect to the generalized distance, which can be of interest to the broader hypothesis testing community.

%\subsection{Proof for  R\'enyi DP}\label{sec.intrordp}
%
%
%
%
%R\'enyi differential privacy (RDP)  \cite{mironov2017renyi} is
% %and Concentrated differential privacy (CDP) \cite{dwork2016concentrated,bun2016concentrated} are 
%based on R\'enyi divergence between the output distributions of $\mathcal{M}$ on the two neighboring datasets.
%
%\begin{definition}[R\'enyi differential privacy (RDP) \cite{mironov2017renyi}]
%	A randomized algorithm $\mathcal{M}: \mathcal{X} \rightarrow \mathcal{R}$ is \emph{$(\alpha,\eps)$-RDP} if for every pair of neighboring datasets $x, x'\in \mathcal{X}$,
%	$$D_\alpha(\mathcal{M}(x) || \mathcal{M}(x'))\le \eps.$$
%\end{definition}
%
%
%%\begin{definition}[zero-Concentrated Differential Privacy (zCDP) \cite{bun2016concentrated}]
%%	A randomized algorithm $\mathcal{M}: \mathcal{X} \rightarrow \mathcal{R}$ is \emph{$(\xi,\rho)$-zCDP} if for every pair of neighboring datasets $x, x'\in \mathcal{X}$, and for all $\alpha\in(1,\infty)$,
%%	$$D_\alpha(\mathcal{M}(X) || \mathcal{M}(X'))\le \xi +\rho \alpha.$$
%%\end{definition}
%
%
%R\'enyi divergence has the chain rule property, similar to KL divergence in Equation \ref{chain.KL} (which is the case $\alpha=1$). However, 
%%we show that it does not satisfy the coupling property (see Section \ref{sec.concompddp}), 
% it does not satisfy the coupling property, 
%and that Theorem \ref{thm.reduction} does not hold for  R\'enyi DP. Thus, proving Theorem \ref{thm.rdp} requires a different approach. 
%
%%\sv{why do we index from $1$ to $k$ here but $0$ to $k-1$ elsewhere?  would be better to be consistent, though not urgent for the SODA submission}	
%First, we reformulate Theorem~\ref{thm.rdp} as follows:
%\begin{theorem} \label{thm.rdp-sum}
%	For all $\alpha>1$, $k\in \mathbb{N}$, $\eps_1,\ldots, \eps_k>0$, and all interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ such that $\mathcal{M}_i$ is $(\alpha,\eps_i)$-RDP for $i=1,2 \ldots, k$, 
%	the concurrent composition $\concomp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ of interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ is $(\alpha,\sum_{i=1}^k\eps_i)$-RDP.
%\end{theorem}
%The reason that Theorem~\ref{thm.rdp-sum} is equivalent to Theorem~\ref{thm.rdp} is that when the order $\alpha$ of the R\'enyi divergence is fixed, then summing the $\eps_i$'s is the optimal composition bound for RDP \cite{mironov2017renyi}. 
%%\sv{citation?}
%
%To prove a summation bound like the above, it is tempting to use a {\em hybrid argument} and argue via a triangle inequality that:
%\begin{align*}
%	D_\alpha(\View(B\leftrightarrow &(\mathcal{M}_1(x), \ldots, \mathcal{M}_{k}(x))) || \View(B\leftrightarrow (\mathcal{M}_1(x'), \ldots, \mathcal{M}_{k}(x'))) ) \\
%	\leq \sum_{i=1}^{k} D_\alpha ( 
%	&\View(B\leftrightarrow 
%	(\mathcal{M}_1(x'), \ldots, \mathcal{M}_{i-1}(x'), \cM_{i}(x), \cM_{i+1}(x), \ldots,\cM_k(x)))\\
%	|| 
%	&\View(B\leftrightarrow 
%	(\mathcal{M}_1(x'), \ldots, \mathcal{M}_{i-1}(x'), \cM_{i}(x'), \cM_{i+1}(x), \ldots,\cM_k(x)))
%	).
%\end{align*}	
%
%That is, we change the inputs to the mechanisms from $x$ to $x'$ one at a time.
%The hybrids in the $i$'th term differ only in the input to mechanism $i$, so the R\'enyi divergence can be bounded by $\eps_{i}$.  Unfortunately, R\'enyi divergence does {\em not} satisfy a triangle inequality (except when $\alpha=\infty$).  Nevertheless,
%we prove the following similar statement for the setting of concurrent interactions that suffices:
%
%\begin{lemma}\label{lemma.triangle}
%	For every adversary $B$ concurrently interacting with interactive RDP mechanisms $\mathcal{M}_1, \mathcal{M}_2, \ldots, \mathcal{M}_k$ operating on two neightboring datasets $x, x'$, we have
%	%it is equivalent to consider a set of hybrid experiments where we compare $(M_1(x), \ldots, M_{j-1}(x), M_j(x), M_{j+1}(x), \ldots, M_k(x))$ to \\ $(M_1(x), \ldots, M_{j-1}(x), M_j(x'), M_{j+1}(x), \ldots, M_k(x))$, that is 
%	%the $\alpha$-R\'enyi divergence between the adversary $B$'s views on two neighboring datasets $x,x'$ satisfies
%	\begin{align*}
%		&D_\alpha( \View(B\leftrightarrow (\mathcal{M}_1(x), \ldots, \mathcal{M}_{k}(x))) || \View(B\leftrightarrow (\mathcal{M}_1(x'), \ldots, \mathcal{M}_{k}(x'))) ) \\
%		=&\sum_{i=1}^k D_\alpha ( \View(B\leftrightarrow (\mathcal{M}_1(x), \ldots, \mathcal{M}_{k}(x))) || \View(B\leftrightarrow (\mathcal{M}_1(x), \ldots, \mathcal{M}_{i-1}(x), \mathcal{M}_i(x'), \mathcal{M}_{i+1}(x), \ldots, \mathcal{M}_{k}(x)))),
%	\end{align*}
%\end{lemma}
%%\sv{fixed indexing from $j$ to $i$ in lemma statement}
%where $\View(B\leftrightarrow 
%(\mathcal{M}_1(x'), \ldots, \mathcal{M}_{i-1}(x'), \cM_{i}(x'), \cM_{i+1}(x), \ldots,\cM_k(x)))$ is defined similarly to $\View(B \leftrightarrow \concomp(\mathcal{M}_1, \ldots, \mathcal{M}_k)(x))$, except that we give mechanism $\mathcal{M}_j$ input $x'$ rather than input $x$.
%In contrast to the hybrid argument approach, here we always compare the case that all of the inputs are $x$ to the case where one input is $x'$.  Still, the fact that in the $i$'th term, the inputs only differ in the input to mechanism $\cM_i$ allows us to still obtain a bound of $\sum_i \eps_i$.
%
%\iffalse
%Lemma \ref{lemma.triangle} decomposes the R\'enyi divergence of the adversary's views of the concurrent composition on operating on $x,x'$ into a set of R\'enyi divergence of ``hybrid experiments'' where we compare $(\mathcal{M}_1(x), \ldots, \mathcal{M}_{j-1}(x), \mathcal{M}_j(x), \mathcal{M}_{j+1}(x), \ldots, \mathcal{M}_k(x))$ to $(\mathcal{M}_1(x), \ldots, \mathcal{M}_{j-1}(x), \mathcal{M}_j(x'), \mathcal{M}_{j+1}(x), \ldots, \mathcal{M}_k(x))$. In each experiment, only $\mathcal{M}_j$ operates on $x'$ with all other mechanisms operating on $x$, which is different from a standard ``hybrid experiments'' where we incrementally have one more mechanism operating on $x'$.  We note that R\'enyi divergence in general does not satisfy a triangle inequality.
%
%Lemma \ref{lemma.triangle} implies that if $\mathcal{M}_j$ is $(\alpha,\eps_j)$-RDP, then the $j$th term in the above summation is bounded by $\eps_j$, so the summation is bounded above by $\sum_j \eps_j$, which is the tight bound for composition of non-interactive RDP mechanisms. We provide the detailed proof in Section \ref{sec.RDP}.
%\fi

%Lemma \ref{lemma.triangle} decomposes the privacy of the concurrent composition of $M_1, M_2, \ldots, M_k$ into the summation of the privacy of each individual mechanism conditioned on all other mechanisms with input $x$. Hence, the privacy also adds up for $\concomp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$. We provide the detailed proof in Section \ref{sec.RDP}.


%we provide tools to analyze KL-divergence and R\'enyi divergence, and show that any composition theorems for non-interactive R\'enyi DP mechanisms also extend to the concurrent composition of interactive  R\'enyi DP mechanisms.




\subsection{Independent Work by Lyu}
%\sv{moved this discussion here and edited it}

In independent and concurrent work, Lyu~\cite{lyu2022composition} proves Theorem \ref{thm.concomp} with a different argument.  They show
that every interactive $(\eps,\delta)$-DP mechanism can be simulated by interactive post-processing of a non-interactive $(\eps,\delta)$-DP mechanism, via an argument that is specific to $(\eps,\delta)$-DP that does not seem to generalize to arbitrary tradeoff functions $f$.  Indeed, they leave the the general case of $f$-DP as an open problem, which is solved by our Theorems~\ref{thm.fdp} and \ref{thm.reduction}.


On the other hand, Lyu~\cite{lyu2022composition} also proves an optimal concurrent composition theorem for R\'enyi DP of any fixed order. In an earlier version of our paper~\cite{vadhan2022concurrent}, we also claimed such a result, but our proof was incorrect (except for the case of R\'enyi DP of order $\alpha=1$),\footnote{Specifically, we stated and used a chain rule for R\'enyi divergence that only holds for order $\alpha=1$ (i.e. KL divergence).} as pointed out to us by Lyu. In this revision, we give a simple proof of Lyu's theorem for R\'enyi DP by characterizing the optimal adversary strategy in Section \ref{sec.RDP}.


	


==> Arxiv version/mainbody.tex <==
%!TEX root = main.tex

\section{Generalized Definitions of DP Mechanisms}\label{sec.dDP}


%We introduce the generalized notion of differential privacy $d$-DP with respect to $\mathcal{D}$ based a generalized distance measure that consists of a complete partially ordered set (poset) $(\mathcal{D},\preceq)$ and a mapping $D$ that maps a pairs of random variables $X$ and $Y$ to an element of the complete partially ordered set $\mathcal{D}$.  The generalized distance should obey several properties.

To prove our results and discuss the several variants of differential privacy, it is convenient to introduce a more general abstraction, where distances between probability distributions can be in an arbitrary partially ordered set.

%\wz{``taking values in the same set'' is a little unclear, since it suggests they have the same support. Technically speaking, I suppose you mean they are random variables over the same sigma field, but I understand you might want to not get into that terminology unnecessarily.}

\begin{definition}[Generalized probability distance]
	A {\em generalized probability distance measure} is a tuple $(\mathcal{D}, \preceq, D)$ such that
	\begin{enumerate}
		\item $(\mathcal{D}, \preceq)$ is a partially ordered set (poset).
		\item $D$ is a mapping that takes any two random variables $X,X'$ over the same measurable space to an element $D(X,X')$ of $\mathcal{D}$.
		\item (Post-processing.) The generalized distance mapping $D$ is closed under post-processing, meaning that for every function $g$, $D(g(X), g(X'))\preceq D(X,X')$.
		\item (Joint Convexity.)  Suppose we have a collection of random variables $(X_i, X'_i)_{i\in \mathcal{I}}$ and a random variable $I$ distributed on $\mathcal{I}$. If $D(X_i, X'_i) \preceq d$ for all $i\in \mathcal{I}$, then $D(X_I, X'_I) \preceq d$.
	\end{enumerate}
\end{definition}


For the generalized notion $d$-$\mathcal{D}$ DP, the difficulty of distinguishing two neighboring datasets is measured by the generalized distance between the distributions of an adversary's views. The partially ordered set allows us to compare the level of privacy guarantees of mechanisms.


%In this section, we show that interactive hypothesis testing can be reduced to non-interactive hypothesis testing. We prove a general result for an generalized notion of differential privacy $d$-$\mathcal{D}$ DP based a generalized distance measure that consists of a partially ordered set $(\mathcal{D},\preceq)$ and a mapping $D$ that maps a pairs of random variables $X$ and $Y$ to an element of the partially ordered set $\mathcal{D}$. The difficulty of distinguishing two neighboring databases is measured by the generalized distance between the distributions of an adversary's views. Furthermore, the generalized distance should obey several properties.

\begin{definition}[$d$-$\mathcal{D}$ DP]\label{def.ddp}
	Let $(\mathcal{D}, \preceq, D)$ be a generalized probability distance.
	For $d \in \mathcal{D}$, we call an interactive mechanism $\mathcal{M}$ {\em $d$-$\mathcal{D}$ DP} if for every adversary $B\in \mathcal{B}$ and every pair of neighboring datasets $x,x'$, we have 
	$$D(\View ( B \leftrightarrow \mathcal{M}(x))   ,\View (B \leftrightarrow \mathcal{M}(x') )) \preceq d.$$ 
\end{definition} 

%The partially ordered set allows us to compare the level of privacy guarantees of a mechanism, and the mapping captures a distance metric. 

Let us instantiate the standard pure DP and its variants using the definition above by specifying the generalized distances.


\paragraph{Example: pure DP.} For pure DP,  a smaller $\eps$ provides stronger privacy guarantee, so the partially ordered set  $\mathcal{D}$ is defined as $((\mathbb{R}^{\ge0})\cup \{\infty\}, \le)$. 
%It is easy to see $((\mathbb{R}^ \ge0)\cup \{\infty\}, \le)$ is complete. 
The distance mapping is the max-divergence $D_\infty$.  For two probability distributions $P$ and $Q$, the max-divergence is $$D_\infty(P||Q):=\sup_{T\subset \supp(P)}\log \left(  \frac{\Pr(P(x)\in T)}{\Pr(Q(x)\in T)} \right) .$$
Max-divergence is closed under post-processing due to the data-processing inequality. Max-divergence satisfies joint convexity due to the following lemma.
\begin{lemma}[\cite{van2014renyi}]\label{lemma.convex}
	For every two pairs of probability distributions $(P_0, Q_0)$ and $(P_1, Q_1)$, and every $\lambda\in (0,1)$, 
	\begin{equation*}
		D_\infty((1-\lambda) P_0+\lambda P_1 || (1-\lambda) Q_0+Q_1)\le \max \{ D_\infty(P_0||Q_0) , D_\infty(P_1||Q_1) \}.
	\end{equation*}
\end{lemma}


\paragraph{Example: R\'enyi DP} For R\'enyi DP of order $\alpha$, the partially ordered set $\mathcal{D}$ is also $((\mathbb{R}^{\ge0})\cup \{\infty\}, \le)$. The distance mapping is $\alpha$-R\'enyi divergence for $\alpha\in(1, \infty)$. 
The R\'enyi divergence is defined as follows.
\begin{definition}[R\'enyi divergence \cite{renyi1961measures}]
	For two probability distribution $P$ and $Q$, the R\'enyi divergence of order $\alpha>1$ is 
	\begin{equation*}
		D_\alpha(P||Q)=\frac{1}{\alpha-1}\log \left(\mathrm{E}_{x\sim Q} \left[\left(\frac{P(x)}{Q(x)}\right)^\alpha\right]\right).
	\end{equation*}
\end{definition}
R\'enyi divergence is also closed under post-processing due to the data-processing inequality, and it satisfies the joint convexity because an analogue of Lemma \ref{lemma.convex} also holds for R\'enyi divergence:

\begin{lemma}[\cite{van2014renyi}]
	For every order $\alpha>1$, every two pairs of probability distributions $(P_0, Q_0)$ and $P_1, Q_1$, and every $\lambda\in (0,1)$, 
	\begin{equation*}
		D_\alpha((1-\lambda) P_0+\lambda P_1 || (1-\lambda) Q_0+Q_1)\le \max \{ D_\alpha(P_0||Q_0) , D_\infty(P_1||Q_1) \}.
	\end{equation*}
\end{lemma}



\paragraph{Example: $f$-DP.} For $f$-DP, the partially ordered set  $\mathcal{D}$ is defined as $(\mathcal{F}, \preceq)$, where $\mathcal{F}$ is the set of all trade-off functions that satisfies the conditions in Proposition \ref{def.tradeoffclass}. The partial ordering is defined as $f_1\preceq f_2$ if  $f_1(\alpha)\ge f_2(\alpha)$ holds  for all $\alpha \in [0,1]$. Note that the direction of the inequalities is reversed, corresponding to the fact that a larger trade-off function means less privacy loss. The distance mapping is the trade-off function $T$ in Definition \ref{tradeoff.def}.

$f$-DP also satisfies the two properties. First, $f$-DP is preserved under post-processing. We will only need to show the joint convexity of $f$-DP. 

\begin{lemma}
	Suppose we have a collection of random variables $(X_i, X'_i)_{i\in \mathcal{I}}$ and a random variable $I$ distributed on $\mathcal{I}$. If $T(X_i, X'_i)\ge f$ for all $i\in \mathcal{I}$, then $T(X_I, X'_I)\ge f$.
\end{lemma}

\begin{proof}
	%Define $D(X_i, X'_i)\le d$ if the tradeoff function satisfies $T(X_i, X'_i)\ge f_d$. 
	For any random variable $I$ distributed on $\mathcal{I}$.  We have
	\begin{align}
		\MoveEqLeft	T(X_I, X'_I)(\alpha)=\inf_{\phi} \left\lbrace  \mathrm{E}\left[ 1-\phi(X'_I)  \right] :  \mathrm{E}[\phi(X'_I)]\le \alpha   \right\rbrace   \notag \\
		&=\inf_{\phi}\left\lbrace \mathrm{E}_{i\sim I} \mathrm{E} [1-\phi(X'_i)]:  \mathrm{E}_{i\sim I} \mathrm{E}[\phi(X_i)]\le \alpha  \right\rbrace  \notag  \\
		&\ge \inf_{\phi} \left\lbrace   \mathrm{E}_{i\sim I} [f(\mathrm{E}[\phi(X_i)]  )]:     \mathrm{E}_{i\sim I} \mathrm{E}[\phi(X_i)]\le \alpha      \right\rbrace  \tag{$f$ non-decreasing}  \\
		&\ge \inf_{\phi} \left\lbrace f(\mathrm{E}_{i\sim I} \mathrm{E}[\phi(X_i)]  ): \mathrm{E}_{i\sim I} \mathrm{E}[\phi(X_i)]\le \alpha      \right\rbrace  \tag{$f$ convex}  \\
		&= f(\alpha). \notag
	\end{align}
	Therefore, we have $T(X_I, X'_I)\ge f$. 
\end{proof}

It is useful to work with distance posets that are {\em complete}:
\begin{definition}[Complete poset]
	A partially ordered set (poset) $(\mathcal{D}, \preceq)$ is {\em complete} if for every nonempty subset $S \subseteq \mathcal{D}$ has a supremum $\sup(S)$, where $s \preceq \sup(S)$ for every $s \in S$, and $\sup(S)\preceq t$ for every $t$ satisfying $s \preceq t$ for every $s \in S$.  
\end{definition}

We note that $\sup(S)$ is always unique. The poset $((\mathbb{R}^{\ge0})\cup \{\infty\}, \le)$ used in pure DP and R\`enyi DP is complete by the usual completeness of the real numbers. For the poset $(\mathcal{F}, \preceq)$ used in $f$-DP, we prove it below. Note that if $(\mathcal{D}, \preceq)$ is complete then in Definition \ref{def.ddp} we can take $d=\sup_B D(\View ( B \leftrightarrow \mathcal{M}(x))   ,\View (B \leftrightarrow \mathcal{M}(x') ))$ as the optimal privacy loss for a given interactive mechanism $\mathcal{M}$.

%To show $f$-DP is an example of $d$-DP wrt.$\mathcal{D}$, we first show that the partially ordered set $(\mathcal{F}, \preceq)$ is complete. 


\begin{lemma}\label{lemma.complete}
	The partially ordered set $(\mathcal{F}, \preceq)$, where $\mathcal{F}$ consists of all trade-off functions satisfying the conditions in Proposition \ref{def.tradeoffclass}, is complete. Specifically, for $S \subseteq \mathcal{F}$, $\sup S$ is a trade-off function defined as follows.
	\begin{equation}
	\sup S = h(\alpha) :=\inf_{\substack{F: \supp(F)\subseteq S \\ A: S\rightarrow [0,1]}} \left\lbrace \mathrm{E}[F(A(F))]: \mathrm{E}[A(F)]\le \alpha \right\rbrace,
	\end{equation}
	where $F$ is a random variable that takes value in $S$ and $A: S\rightarrow [0,1]$ is a function. 
\end{lemma}

%\todo{comment this out. but for future. $A$ measurable function.}

%The proof of Lemma \ref{lemma.complete} relies on the following property of trade-off functions.
%
%\begin{proposition}\label{prop.sup}
%	The supremum of trade-off functions $f$ and $g$ is as follows.
%	\begin{equation}\label{eq.sup}
	%		h(\alpha):=\sup(f, g)=\inf_{p,\alpha_1,\alpha_2} \left\lbrace  pf(\alpha_1)+(1-p)g(\alpha_2): p\alpha_1+(1-p)\alpha_2=\alpha  \right\rbrace .
	%	\end{equation}
%\end{proposition}

\begin{proof}
	We first show that $h$ is the least upper bound for $S$. We shall show that for any tradeoff function $h'$ such that $f \preceq h' $ for every $f\in S$, we have $h \preceq h' $. Let $F$ be a random variable such that $\supp(F)\subseteq S$, and let $A: S\rightarrow [0,1]$ be a function such that $ \mathrm{E}[A(F)] \le \alpha$. As stated in Proposition \ref{def.tradeoffclass}, a trade-off function is convex and non-increasing, so by Jensen's inequality, we have 
	\begin{equation*}
		h'(\alpha)\le h'(\mathrm{E}[A(F)]) \le \mathrm{E}[h'(A(F))].
	\end{equation*}
	By the definition of the partial ordering, we have $h'(\alpha)\le f(\alpha)$ for every $\alpha \in [0,1]$ and every $f\in S$, so $ \mathrm{E}[h'(A(F))]\le  \mathrm{E}[F(A(F))]$. Therefore, we have 
	\begin{equation*}
		h'(\alpha)\le \mathrm{E}[F(A(F))],
	\end{equation*}
	Taking the infimum over $F$ and $A$ on both sides, we get $h'(\alpha)\le h (\alpha)$, and therefore, $h\preceq h'$.
	
	Next, we shall show that $h$ is a trade-off function. Following the proposition \ref{def.tradeoffclass}, it suffices to check the four properties for $h$. We begin with proving the convexity of $h$.
	For every $a, b\in[0,1]$, and every $\lambda\in[0,1]$, we have 
	\begin{align}
		h (\lambda a + (1-\lambda) b)=&\inf_{F, A} \left\lbrace  \mathrm{E}[F(A(F))]: \mathrm{E}[A(F)]\le \lambda a + (1-\lambda) b \right\rbrace \notag \\
		\le &\lambda \inf_{F, A} \left\lbrace  \mathrm{E}[F(A(F))]: \mathrm{E}[A(F)]\le a \right\rbrace  
		+(1-\lambda)\inf_{F, A} \left\lbrace  \mathrm{E}[F(A(F))]: \mathrm{E}[A(F)]\le  b \right\rbrace    \label{ineq.1}\\
		=& \lambda h(a) + (1-\lambda) h(b).\notag
	\end{align}
	where inequality \eqref{ineq.1} is because that for every $A_a,F_a$ that satisfies $\mathrm{E}[A(F)]\le a$ and every $A_b,F_b$ that satisfies $\mathrm{E}[A(F)]\le b$, the linear combination $A(F)=\lambda A_a(F_a)+(1-\lambda)A_b(F_b)$ satisfies $\mathrm{E}[A(F)]\le \lambda a + (1-\lambda) b $.  
	Thus, $h$ is convex. $h$ is non-increasing and continuous on $[0,1]$ due to the monotonicity and continuity of $f\in \mathcal{F}$ (Proposition \ref{def.tradeoffclass}). Finally, since $f(x)\le 1-x$ for every $f\in \mathcal{F}$, we have 
	$$h(\alpha)\le \mathrm{E}[F(A(F))] \le \mathrm{E}[1-A(F)] \le 1-\alpha.$$
	Therefore, $h$ is a trade-off function, and $\sup S$ exists.
	%Last, we shall show the continuity of $h$. Convexity implies continuity in $(0,1)$ and $h(\alpha)\ge 0$ and $f(\alpha)\le 1-\alpha$ implies continuity at $1$ \cite{dong2019gaussian}, it suffices to show the continuity at $\alpha=0$. Suppose a sequence $\alpha_n\rightarrow 0$. Without loss of generality we can assume $\alpha_n$ is decreasing. 
	
\end{proof}



A convenient consequence of joint convexity is that it suffices to consider deterministic adversaries.

\begin{lemma}\label{lemma.det}
	An interactive mechanism $\mathcal{M}$ is $d$-$\mathcal{D}$ DP, if and only if for every pair of neighboring datasets $x,x'$, for every deterministic adversary algorithm $B$, we have $D(\View ( B, \mathcal{M}(x))   ,\View (B, \mathcal{M}(x') )) \preceq d$. 
\end{lemma}

\begin{proof}
	The necessity is immediately implied by Definition \ref{def.ddp}. We shall prove the sufficiency. Let $B$ be a randomized adversary.  If we fix the coin tosses of
	$B$ to a value $r$, we obtain a deterministic adversary $B_r$.
	By hypothesis, we have $D(\View ( B_r, \mathcal{M}(x))   ,\View (B_r, \mathcal{M}(x') )) \preceq d$.  Now let random variable $R$ be uniformly distributed over the coins of $A$.  Then the view of the randomized adversary $B$ when interacting with $\mathcal{M}$ consists of the coins $R$ and the view of the deterministic adversary $B_R$.  That is,
	$$\View ( B \leftrightarrow \mathcal{M}(x)) = (R, \View(B_R\leftrightarrow \mathcal{M}(x))),$$
	and similarly for $x'$. 
	By joint convexity, we deduce:
	$$\View ( B \leftrightarrow \mathcal{M}(x)) \preceq d.$$
	%	\wz{check my definition of the view.} \sv{I edited the proof.  in future version, should elaborate on the application of joint convexity in the last step}
\end{proof}


%To obtain our main results for $f$-DP (Theorems \ref{thm.fdp} and \ref{thm.reduction}), we prove the following general theorems about $d$- $\mathcal{D}$ DP in Section \ref{sec.concompddp}.


%\begin{theorem}[Theorem \ref{thm.fdp} generalized]\label{thm.concomp_d}
%	Suppose that the generalized probability distance $(\mathcal{D}, \preceq, D)$ satisfies the chain rule, every $d\in \mathcal{D}$ satisfies the coupling property, and $(\mathcal{D}, \preceq)$ is complete. Suppose for all non-interactive mechanism $\mathcal{M}_1, \ldots, \mathcal{M}_k$ such that $\mathcal{M}_i$ is $d_i$-$\mathcal{D}$ DP for $i=1,2 \ldots, k$, their composition $\comp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ is $d$-$\mathcal{D}$ DP, then the concurrent composition $\concomp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$  of interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ such that $\mathcal{M}_i$ is $d_i$-$\mathcal{D}$ DP is also $d$- $\mathcal{D}$ DP.
%\end{theorem}



\section{Coupling and Chain Rule Properties of $f$-DP}

In this section, we prove that $f$-DP has the coupling and chain rule properties that we use to prove Theorems \ref{thm.fdp} and \ref{thm.reduction}.


%To prove Theorem \ref{thm.concomp_d}, we first prove a result that reducing an interactive $d$-$\mathcal{D}$ DP mechanism to a non-interactive interactive $d$-$\mathcal{D}$ DP mechanism in Theorem \ref{thm.post_gen}. We additionally require the coupling property in Definition \ref{def.couplingP} and the chain rule property in Definition \ref{def.chain}. The coupling property ensures that there exists a  $d$-$\mathcal{D}$ DP mechanism $\mathcal{M}'$ that dominates among all other  $d$-$\mathcal{D}$ DP mechanisms. For any interactive $d$-$\mathcal{D}$ DP mechanism, we denote $X_i$ as the random output in the $i$th round of interaction, and $Y$ is the random output of mechanism $\mathcal{M}'$. The chain rule property ensures that for every pair of random variables $Y$ and $Y'$ where $Y$ is jointly distributed with $X$ and $Y'$ is jointly distributed with $X'$, the distance between $(X,Y)$ and $(X',Y')$ can be fully determined by a set of distances between $Y$ and $Y'$ conditioned on $X$ and $X'$ taking value $x \in supp(X) \cap supp(X')$.

\begin{definition}[Coupling property]\label{def.couplingP}
	We say that a generalized distance $D$ has the {\em coupling property} if for any two pairs of random variable $X,X'$ and $Y,Y'$,  we have $D(X, X') \preceq d$ and $D(Y, Y') \preceq d$, then there exists a coupling of $X$ and $Y$ (denoted as $(X,Y)$), and a coupling of $X'$ and $Y'$ (denoted as $(X',Y')$), such that $D((X,Y),(X',Y')) \preceq d$.
\end{definition}

%In the following lemma, we show that $f$-DP has the coupling property. 

\begin{lemma}[Lemma \ref{lemma.coupling} restated]\label{lemma.coupling2}
	$(\mathcal{F}, \preceq, T)$ has the coupling property: Suppose $f$ is a trade-off function and
	we have random variables $X$, $Y$  and $X'$, $Y'$ such that 
	\begin{equation*}
		T(X,X') \ge f \quad \text{and} \quad T(Y,Y')\ge f.
	\end{equation*}
	Then there exists couplings $(X,Y)$ and $(X',Y')$ such that
	\begin{equation*}
		T((X,Y)||(X',Y'))\ge f.
	\end{equation*}
\end{lemma}


We prove this lemma using the following result:

\begin{theorem}[Blackwell Theorem \cite{dong2019gaussian} (also see \cite{blackwell1953equivalent, kairouz2015composition})]
	Let $P, Q$ be probability distributions on $X$ and $P', Q'$ be probability distributions on $Y$. The following two statements are equivalent:
	\begin{enumerate}
		\item $T(P,Q) \le T(P',Q')$.
		\item There exists a randomized algorithm $\mathrm{Proc}: X\rightarrow Y$ such that $\mathrm{Proc}(P)=P'$ and  $\mathrm{Proc}(Q)=Q'$.
	\end{enumerate}
\end{theorem}



\begin{proof}[Proof of Lemma \ref{lemma.coupling2}]
	
	Since a function is called a trade-off function if it is equal to $T(P,P')$ for some distribution $P$ and $P'$, for a given rade-off function $f$, there exists a pair of random variables $P, P'$  such that $T(P, P')=f$. 
	%By Proposition 2.2 in \cite{dong2019gaussian}, for a given trade-off function $f$, there exists a pair of random variables $P, P'$  such that $T(P, P')=f$. 
	By the Blackwell Theorem, since $T(P, P')=f\le T(X, X')$, there exists a randomized algorithm $\mathcal{P}_0$ such that $\mathcal{P}_0(P)$ and  $\mathcal{P}_0(P')$ are identically distributed to $X$ and  $X'$, respectively. Similarly, since $T(P, P')=f\le T(Y, Y')$, there exists a randomized algorithm $\mathcal{P}_1$ such that $\mathcal{P}_1(P), \mathcal{P}_1(P')$ is identically distributed to $Y, Y'$, respectively. We construct a coupling of $X$ and $Y$ as $(\mathcal{P}_0(P), \mathcal{P}_1(P))$, and  a coupling of $X'$ and $Y'$ as $(\mathcal{P}_0(P'), \mathcal{P}_1(P'))$. Then the trade-off function between the two couplings satisfies the following inequality.
	\begin{align}
		&T((\mathcal{P}_0(P), \mathcal{P}_1(P)), (\mathcal{P}_0(P'), \mathcal{P}_1(P')))  \notag \\
		&\ge T(P,P') \label{eq2} \\
		&=f,
	\end{align}
	where Equation \eqref{eq2} follows from Lemma 2.9 in \cite{dong2019gaussian}, completing the proof.
\end{proof}

To formally state the chain rule property, we need a couple of definitions.

%\begin{definition}
%	If $(\mathcal{D},\preceq)$ is a poset, and $S$ is a finite set, then $(\mathcal{D}^S,\preceq)$ is the poset defined by $( (a)_{s\in S}) \preceq ( (b)_{s\in S}) $ if $a_s \preceq b_s$ for every $s\in S$. 
%\end{definition}

%\todo{ask Salil to take a look. put continuity with respect to a poset, monotone should be more general for poset}



\begin{definition}[Continuous function]\label{def.conf}
	Let $(A, \preceq)$ and $(B, \preceq)$ be complete posets. A function $f: A\rightarrow B$ is {\em continuous} if $f(\sup(S))=\sup(f(S))$ for every set $S\subseteq A$.
\end{definition}

Observe that every continuous function is monotone: if $a\preceq a'$ are elements of $A$, then $f(a')=f(\sup(a, a'))=\sup(f(a),f(a'))\succeq f(a)$.

\begin{definition}[Continuous in each variable]\label{def.conf2}
	Let $S$ be a finite set and $|S|=n$. Let $(A, \preceq)$ and $(B, \preceq)$ be complete posets. A function $f: A^S\rightarrow B$ is {\em continuous in each variable} if for every $i$, 
	and
	for every $a_1,\ldots, a_{i-1}, a_{i+1}, \ldots, a_n \in A$, 
	the function $g(x)=f(a_1,\ldots,a_{i-1},x,a_{i+1},\ldots,a_n)$ is a continuous function from $A$ to $B$.   
	% we have
	%	\begin{equation*}
		%		f(a_1, \ldots, a_{i-1}, \sup S_i, a_{i+1}, \ldots, a_n)= \sup(f (a_1,\ldots, a_{i-1}, a_i, a_{i+1},\ldots, a_n): a_i\in S_i).
		%	\end{equation*}
	% $f(\sup(S))=\sup(f(S))$ for every set $S$.
\end{definition}

\iffalse
If a function in continuous in each variable, then it is also monotone in each variable:  if $a_{i}\preceq a'_{i}$ are elements of $A$, then 
\begin{align*}
	f(a_1,\ldots, a_{i-1}, a'_i, a_{i+1}, \ldots, a_n)&=f(a_1,\ldots, a_{i-1}, \sup(a, a'),  a_{i+1}, \ldots, a_n)\\
	&=\sup(f(a_1,\ldots, a_{i-1}, x, a_{i+1},\ldots, a_n): x\in (a_i, a'_i)) \\
	&\succeq f(a_1,\ldots, a_{i-1}, a_i, a_{i+1}, \ldots, a_n).
\end{align*}
\fi

\begin{definition}[Chain rule]\label{def.chain}
	We say that a generalized probability distance $(\mathcal{D}, \preceq, D)$ satisfies the chain rule property if
	for every pair of random variables $(X, X')$ on the same domain $\mathcal{X}$, there is a function that is continuous in each variable:
	%that maps from a poset $\mathcal{D}^{\supp(X)\cap \supp(X')}$, which consists of $|\supp(X)\cap \supp(X')|$ elements, to a element in the poset $\mathcal{D}$: 
	$ \mathrm{ChainRule}_{X,X'}: \mathcal{D}^{\supp(X)\cap \supp(X')}\rightarrow \mathcal{D}$ such that for every pair of random variables $Y$ and $Y'$ where $Y$ is jointly distributed with $X$ and $Y'$ is jointly distributed with $X'$, we have
	$$D((X,Y),(X',Y')) = \mathrm{ChainRule}_{X,X'}((D(Y|X=x,Y'|X'=x)_{x \in \supp(X) \cap \supp(X')}).$$
\end{definition}

As an example, the standard chain rule of KL divergence is as follows.
\begin{align*}
	D_{\mathrm{KL}}((X,Y)||(X',Y'))&=D_{\mathrm{KL}}(X||X')+D_{\mathrm{KL}}(Y|X|| Y'|X')\\
	&=D_{\mathrm{KL}}(X||X')+\mathrm{E}_{x\sim X}D_{\mathrm{KL}}(Y|X=x|| Y'|X'=x).
\end{align*}
So fixing $X$ and $X'$, we can calculate the KL divergence for arbitrary $Y$ and $Y'$ as a function of the KL divergences $\mathrm{KL}(Y|X=x|| Y'|X'=x)$.


In Lemma \ref{lemma.chain2}, we show that $f$-DP has the chain rule property.

\begin{lemma}[Lemma \ref{lemma.chain} restated] \label{lemma.chain2}
	For every pair of random variables $X, X'$ with finite support, there exists a function that is continuous in each variable $\mathrm{ChainRule}_{X,X'}$ such that for every random variable $Y$ jointly distributed with $X$, and every random variable $Y'$ jointly distributed with $X'$, we have 
	\begin{equation*}
		T((X,Y), (X',Y'))=\mathrm{ChainRule}_{X,X'}((T(Y|X=x, Y'|X'=x)))_{x\in \supp(X)\cap \supp(X') }).
	\end{equation*}
	where $T$ is a trade-off function.
\end{lemma}

%\new{In an earlier version of our paper \cite{vadhan2022concurrent}, we erroneously claimed that $\mathrm{ChainRule}$ was jointly continuous in all of its variables. Here we correct the statement to continuity in each variable, which is all we need.}

%In Lemma \ref{lemma.chain}, we show that $f$-DP has the chain rule property. Specifically, the ChainRule function is given as 
%\begin{equation*}
%	 \mathrm{ChainRule}_{X,X'}((f_x)_{x\in \supp(X)\cap \supp(X') })=\inf_{\alpha_x\in[0,1]}\{ E_{x\in X'}[f_x(\alpha_x)]: E_{x\in X}[\alpha_x]\le \alpha  \}.
%\end{equation*}


\begin{proof}
	
	\begin{claim}
		The ChainRule function for $f$-DP is given as follows.
		\begin{equation}\label{eq.f_chain}
			\mathrm{ChainRule}_{X,X'}\left( (f_x)_{x\in \supp(X)\cap \supp(X') }\right)(\alpha) =\inf_{\alpha_x\in[0,1]}\left\lbrace  \mathrm{E}_{x\sim X'}[f_x(\alpha_x)]: \mathrm{E}_{x\sim X}[\alpha_x]\le \alpha  \right\rbrace .
		\end{equation}
	\end{claim} 
	
	We first prove this claim.	
	Suppose $Y$ is jointly distributed with $X$, and $Y'$ is jointly distributed with $X'$.  We consider hypothesis tests distinguishing $(X,Y)$ and $(X',Y')$. Let $\phi$ be any decision rule for this testing, $\alpha(\phi)$ and $\beta(\phi)$ be the corresponding Type I error and Type II error, respectively. For a given instance $x \in \supp(X)\cap \supp(X')$, let $\phi_x(y):=\phi(x,y)$. Additionally, let $f_x$ be the trade-off function conditioned on $x$, i.e.,
	
	\begin{equation}\label{def.fx0}
		f_{x}(\alpha):=T(Y|X=x, Y'|X'=x)(\alpha)  . 
	\end{equation}
	The type I error $\alpha_\phi$ and type II error  $\beta_\phi$ are given as 
	\begin{equation*}
		\alpha_\phi=\mathrm{E}[\phi(x,y)]=\mathrm{E}_{x\sim X}\mathrm{E}_{y\sim Y}[\phi_x(y)],
	\end{equation*}
	and 
	\begin{equation*}
		\beta_\phi=1- \mathrm{E}[\phi(x',y')]=1-\mathrm{E}_{x\sim X'} \mathrm{E}_{y'\sim Y'}[\phi_{x'}(y')].
	\end{equation*}	
	For every fixed $x \in \supp(X)\cap \supp(X')$ and every decision rule $\phi$ such that $\mathrm{E}_{y\sim Y}[\phi_x(y)]=\alpha_x$, by the definition of $f_{x}$ in \eqref{def.fx0}, we have 
	\begin{equation*}
		1- \mathrm{E}_{y'\sim Y'}[\phi_{x'}(y')] \ge f_{x}(\alpha_x).
	\end{equation*}
	Therefore, the trade-off function between $(X,Y)$ and $(X',Y')$ satisfies the following inequality:
	\begin{align}
		T((X,Y),(X',Y'))(\alpha)=\inf_\phi \left\lbrace  \beta_\phi:\alpha_\phi\le \alpha  \right\rbrace  &= \inf_\phi \left\lbrace  1-\mathrm{E}_{x\sim X'} \mathrm{E}_{y'\sim Y'}[\phi_{x'}(y')]: \mathrm{E}_{x\sim X}\mathrm{E}_{y\sim Y}[\phi_x(y)]\le \alpha \right\rbrace  \notag \\ 
		&\ge \inf_{\{\alpha_x\}}\left\lbrace \mathrm{E}_{x\sim X'}[f_{x}(\alpha_x)]: \mathrm{E}_{x\sim X}[\alpha_x]\le \alpha \right\rbrace . \label{eq.5}
	\end{align}
	On the other hand, by the definition of $f_{x}$, for every $0<\alpha_x<1$ and $\delta>0$, there exists a decision rule $\phi^\delta$ such that $1- \mathrm{E}_{y'\sim Y'}[\phi^\delta_{x'}(y')]  \le f_{x}(\alpha_{x})+\delta$ and $\mathrm{E}_{y\sim Y}[\phi^\delta_x(y)]\le \alpha_x$. Then we have
	\begin{align*}
		\inf_{\{\alpha_x\}} \left\lbrace \mathrm{E}_{x\sim X'}[f_{x}(\alpha_{x})]: \mathrm{E}_{x\sim X}[\alpha_{x}]\le \alpha \right\rbrace &\ge \inf_\delta \left\lbrace \mathrm{E}_{x\sim X'}[1- \mathrm{E}_{y'\sim Y'}[\phi^\delta_{x'}(y')]-\delta]: \mathrm{E}_{x\sim X}[ \mathrm{E}_{y\sim Y}[\phi^\delta_{x}(y)]]\le \alpha \right\rbrace . \\
		&=\inf_\delta \left\lbrace  \beta_{\phi^\delta}:\alpha_{\phi^\delta}\le \alpha \right\rbrace -\delta \\
		&\ge \inf_\phi \left\lbrace  \beta_{\phi}:\alpha_{\phi}\le \alpha \right\rbrace -\delta \\
		&=T((X,Y),(X',Y'))(\alpha)-\delta.
	\end{align*}
	Let $\delta$ go to $0$, and combining with
	%, the decision function $\phi^\delta$ will converge to the decision rule $\phi^*$ such that the infimum in \eqref{def.fx0} is reached over all the decision rules such that $\mathrm{E}_{y\sim Y}[\phi_x(y)]\le \alpha_x$, and thus, we get
	%\begin{align}\label{eq.6}
	%	\inf \left\lbrace \mathrm{E}_{x\sim X'}[f_{x}(\alpha_{x})]: \mathrm{E}_{x\sim X}[\alpha_{x}]\le \alpha \right\rbrace  &\ge \inf \left\lbrace \mathrm{E}_{x\sim X'}[1- \mathrm{E_{y'\sim Y'}}[\phi^*_{x'}(y')]]: \mathrm{E}_{x\sim X}[\alpha_{x}]\le \alpha \right\rbrace  \notag \\
	%	&= T((X,Y),(X',Y'))(\alpha). 
	%\end{align}
	Equation \eqref{eq.5}, we have
	\begin{equation}\label{eq.7}
		T((X,Y),(X',Y'))(\alpha)=\inf \left\lbrace \mathrm{E}_{x\sim X'}[f_{x}(\alpha_{x})]: \mathrm{E}_{x\sim X}[\alpha_{x}]\le \alpha \right\rbrace .
	\end{equation}
	completing the proof for this claim.
	
	Next, we shall show that the ChainRule function defined in \eqref{eq.f_chain} is continuous in each variable. 
%	By assumption, $\supp(X)\cap \supp(X')$ has finite elements, and we have $X= x_j$ with probability $p_j$ and $X'=x_j$ with probability $p'_j$. We can write the ChainRule function as 
%	\begin{equation}\label{eq.chainrewrite}
%		\mathrm{ChainRule}_{X,X'}\left( (f_x)_{x\in \supp(X)\cap \supp(X')}\right) (\alpha)= \inf_{\alpha_{x_j}\in[0,1]}\left\lbrace  \sum_j p'_j f_{x_j}(\alpha_{x_j}) : \sum_j p_j \alpha_{x_j}\le \alpha  \right\rbrace .
%	\end{equation}
	Our goal is to show that for every $i$, every $S_i \subseteq \mathcal{D}$, and for every $f_1,\ldots, f_{i-1}, f_{i+1}, \ldots, f_n \in \mathcal{D}$, we have
	\begin{equation*}
		\mathrm{ChainRule}_{X,X'}(f_1, \ldots, f_{i-1}, \sup S_i, f_{i+1}, \ldots, f_n )= \sup(\mathrm{ChainRule}_{X,X'} (f_1,\ldots, f_{i-1}, f_i, f_{i+1}, \ldots, f_n): f_i\in S_i).
	\end{equation*}
	%$\mathrm{ChainRule}_{X,X'}(\sup(S))=\sup(\mathrm{ChainRule}_{X,X'}(S))$ for every finite set $S$. 


%	\wz{new version below}
	Let $S=(\mathrm{ChainRule}_{X,X'} (f_1,\ldots, f_{i-1}, f_i, f_{i+1}, \ldots, f_n): f_i\in S_i)$. For every random variable $F$ such that $\supp(F)\subseteq S$, we have $F$ taking values as $\mathrm{ChainRule}_{X,X'} (f_1,\ldots, f_{i-1}, f_i, f_{i+1}, \ldots, f_n): f_i\in S_i$, so it is equivalent to consider a random variable $F_i$ such that $\supp(F_i)\subseteq S_i$. For every function $A: S\rightarrow [0,1]$, we also slightly abuse the notation and use $A(F_i)$ to represent $A(F)$.
	For every $\alpha\in [0,1]$, we have 

	\begin{align}
	\MoveEqLeft	 \sup(\mathrm{ChainRule}_{X,X'} (f_1,\ldots, f_{i-1}, f_i, f_{i+1}, \ldots, f_n): f_i\in S_i)(\alpha) \notag \\
	=&\inf_{\substack{F_i: \supp(F_i)\subseteq S_i \\ A: S\rightarrow [0,1]}} \left\lbrace \mathrm{E}_{F_i}\left[ \mathrm{ChainRule}_{X,X'} (f_1,\ldots, f_{i-1}, F_i, f_{i+1}, \ldots, f_n) (A(F_i)) \right] : \mathrm{E}_{F_i}[A(F_i)]\le \alpha \right\rbrace \tag{by Lemma \ref{lemma.complete}} \\
	=&\inf_{\substack{F_i: \supp(F_i)\subseteq S_i \\ A: S\rightarrow [0,1]}} \left\lbrace \mathrm{E}_{F_i}\left[ \inf_{\substack{A_1,\ldots,A_n \\ A_j: S_i\rightarrow [0,1]  }} \left\lbrace \mathrm{E}_{j\sim X'} \left[ f_{j} (A_j(F_i)) \cdot \mathbb{I}(j\neq i) + F_i( A_i(F_i))\cdot \mathbb{I}(j=i)  \right] :  \mathrm{E}_{j\sim X}[A_j(F_i)]\le A(F_i)   \right\rbrace  \right] :  \right.  \notag \\
  &\left.	 \mathrm{E}_{F_i}[A(F_i)]\le \alpha \right\rbrace \tag{by \eqref{eq.f_chain}} \\
	=&\inf_{\substack{F_i: \supp(F_i)\subseteq S_i \\ A: S_i\rightarrow [0,1] \\ A_j: S_i\rightarrow [0,1] }} \left\lbrace \mathrm{E}_{F_i} \mathrm{E}_{j\sim X'}  \left[f_{j} (A_j(F_i)) \cdot \mathbb{I}(j\neq i) + F_i( A_i(F_i))\cdot \mathbb{I}(j=i)   \right] : \mathrm{E}_{j\sim X}[A_j(F_i)]\le A(F_i),   \mathrm{E}_{F_i}[A(F_i)] \le \alpha \right\rbrace. \label{eq.constraints1}
\end{align}	

We can interchange the expectation and the infimum in Equation~\eqref{eq.constraints1} because $A_j(f_i)$, $j=1, \ldots, n$, are independent across $f_i\in F_i$. We also have that
\begin{align}
	\MoveEqLeft	 \mathrm{ChainRule}_{X,X'}(f_1, \ldots, f_{i-1}, \sup S_i, f_{i+1}, \ldots, f_n )(\alpha) \notag \\
	=&\inf_{\alpha_1,\ldots, \alpha_n}\left\lbrace \mathrm{E}_{j\sim X'}\left[ f_{j} (\alpha_j) \cdot \mathbb{I}(j\neq i) + (\sup S_i)( \alpha_i)\cdot \mathbb{I}(j=i)  \right] :  \mathrm{E}_{j\sim X}[\alpha_j]\le \alpha   \right\rbrace \tag{by \eqref{eq.f_chain}}  \\
	=&\inf_{\alpha_1,\ldots, \alpha_n}\left\lbrace \mathrm{E}_{j\sim X'}\left[ f_{j} (\alpha_j) \cdot \mathbb{I}(j\neq i) + \inf_{\substack{F_i: \supp(F_i)\subseteq S_i \\ A_{i}: S_i\rightarrow [0,1]}}\left\lbrace \mathrm{E}_{F_i}\left[ F_i(A_{i}(F_i))  \right] : \mathrm{E}[A_{i}(F_i)]\le \alpha_i \right\rbrace \cdot \mathbb{I}(j=i)  \right] :  \mathrm{E}_{j\sim X}[\alpha_j]\le \alpha   \right\rbrace \tag{by Lemma \ref{lemma.complete}}  \\
    =&\inf_{\substack{F_i: \supp(F_i)\subseteq S_i \\ A_i: S_i\rightarrow [0,1] \\ \alpha_1, \ldots, \alpha_n }} \left\lbrace \mathrm{E}_{F_i} \mathrm{E}_{j\sim X'}  \left[f_{j} (\alpha_j) \cdot \mathbb{I}(j\neq i) + F_i( A_i(F_i))\cdot \mathbb{I}(j=i)   \right] :  \mathrm{E}_{j\sim X}[\alpha_j]\le \alpha,  \mathrm{E}_{F_i}[A_i(F_i)] \le \alpha_i   \right\rbrace. \label{eq.constraints2}
\end{align}	


The constraints in \eqref{eq.constraints1} are equivalent to the constraints in \eqref{eq.constraints2}, which can be seen as follows. For all $\alpha_j(F_i)$ ($j=1,\ldots, k$, and $F_i\in \supp(S_i)$) satisfy the constraints in \eqref{eq.constraints1}, let $\alpha_j=\mathrm{E}_{F_i}[ A_j(F_i) ]$, then $\alpha_j$ satisfy the constraints in \eqref{eq.constraints2}. On the other hand, for all $\alpha_j$ ($j=1,\ldots, k$) satisfy the constraints in \eqref{eq.constraints2}, let $\alpha_j=\mathrm{E}_{F_i}[ A_j(F_i) ]$, then $\alpha_j(F_i)$ satisfy the constraints in \eqref{eq.constraints1}. Moreover, with $\alpha_j=\mathrm{E}_{F_i}[ A_j(F_i) ]$, we have
\begin{align}
\MoveEqLeft \mathrm{E}_{j\sim X'}  \left[f_{j} (\alpha_j) \cdot \mathbb{I}(j\neq i) \right]  \notag  \\
=&  \mathrm{E}_{j\sim X'}  \left[f_{j} ( \mathrm{E}_{F_i}[ A_j(F_i) ] ) \cdot \mathbb{I}(j\neq i) \right] \notag \\
\le& \mathrm{E}_{j\sim X'}  \mathrm{E}_{F_i}  \left[f_{j} (  A_j(F_i) ) \cdot \mathbb{I}(j\neq i) \right], \label{eq.convex}
\end{align}
where \eqref{eq.convex} is because trade-off functions are convex. Hence, 
\begin{equation*}
\inf_{\substack{F_i: \supp(F_i)\subseteq S_i \\ A_i: S_i\rightarrow [0,1] \\ \alpha_1, \ldots, \alpha_n }} \mathrm{E}_{j\sim X'}  \left[f_{j} (\alpha_j) \cdot \mathbb{I}(j\neq i) \right]  \le \inf_{\substack{F_i: \supp(F_i)\subseteq S_i \\ A: S_i\rightarrow [0,1] \\ A_j: S_i\rightarrow [0,1]  }} \mathrm{E}_{j\sim X'}  \mathrm{E}_{F_i}  \left[f_{j} (  A_j(F_i) ) \cdot \mathbb{I}(j\neq i) \right].
\end{equation*}
On the other hand, by setting $A_j(F_i)=\alpha_j$ for all $F_i\in S_i$, the above equal sign is reached.

Therefore, we have 
\begin{equation*}
	\mathrm{ChainRule}_{X,X'}(f_1, \ldots, f_{i-1}, \sup S_i, f_{i+1}, \ldots, f_n )= \sup(\mathrm{ChainRule}_{X,X'} (f_1,\ldots, f_{i-1}, f_i, f_{i+1}, \ldots, f_n): f_i\in S_i).
\end{equation*}	
	
\end{proof}

\section{Concurrent Composition of $d$-$\mathcal{D}$ DP}\label{sec.concompddp}

%To obtain our main results for $f$-DP (Theorems \ref{thm.fdp} and \ref{thm.reduction}), we prove the following general theorems about $d$- $\mathcal{D}$ DP in Section \ref{sec.concompddp}.

Theorem \ref{thm.post_gen} shows that if the generalized distance satisfies the coupling property in Definition \ref{def.couplingP}  and the chain rule in Definition \ref{def.chain} , then every interactive $d$-$\mathcal{D}$ DP mechanism can be simulated by an interactive post-processing of a non-interactive $d$-$\mathcal{D}$ DP mechanism. This is a generalized statement of Theorem \ref{thm.reduction}, as $f$-DP is an example of $d$-$\mathcal{D}$ DP.

\begin{theorem}[Theorem \ref{thm.reduction} generalized]\label{thm.post_gen}
	
	Assume that the generalized probability distance measure $(\mathcal{D}, \preceq, D)$ satisfies 
	\begin{enumerate}
		\item $(\mathcal{D}, \preceq)$ is complete.
		\item $\mathcal{D}$ satisfies the chain rule.
		\item every $d\in \mathcal{D}$ satisfies the coupling property.
	\end{enumerate}
	Then for every $d\in 
	\mathcal{D}$ and every interactive $d$-$\mathcal{D}$ DP mechanism $\mathcal{M}$ with finite communication complexity, and every pair of two neighboring datasets $x$ and $x'$, there exists a pair of random variables $Y, Y'$ and an randomized interactive post-processing mechanism $\mathcal{P}$ such that $D(Y, Y')\preceq d$, and for every adversary $B\in \mathcal{B}$, we have
	
	\begin{align}
		\View(B\leftrightarrow \mathcal{M}(x))&\equiv \View(B \leftrightarrow \mathcal{P}(Y))\\
		\View(B \leftrightarrow \mathcal{M}(x'))&\equiv \View(B \leftrightarrow \mathcal{P}(Y')).
	\end{align}
	
\end{theorem}


%From the hypothesis testing perspective, the output of the non-interactive mechanism can be interpreted as the hypothesis testing decision: failing to reject the null hypothesis that the dataset is $x$ for $b=0$, and rejecting the null hypothesis/accepting the alternative hypothesis that the dataset is $x'$ for $b=1$. 

Note that the theorem is stated for mechanisms with {\em finite communication}, which is formally defined as follows.

\begin{definition}
	Let $(A, B)$ be an interactive protocol (as in Definition \ref{def.protocol}). 	We say that $A$ has {\em finite communication} if for every $x_A$ there is a constant $c$, such that for all $r_A, m_1, \ldots, m_{i-1}$, we have 
	\begin{enumerate}
		\item If $\max \{i, |m_1|, \ldots, |m_{i-1}|\}>c$, then $A(x_A, m_1, m_3, \ldots, m_{i-1}; r_A)=\texttt{halt}$.
		\item If $\max \{i, |m_1|, \ldots, |m_{i-1}|\}\le c$, then $ \sum_{j=0}^{i-1} \left| A(x_A, m_1, m_3, \ldots, m_j; r_A)\right| \le c$. 
	\end{enumerate}
	Here $|y|$ denotes the bit length of string $y$. $B$ having finite communication is defined symmetrically.
\end{definition}




%\sv{this proof header should say ``Proof of Theorem 4.1''}

\begin{proof}[Proof of Theorem \ref{thm.post_gen}]
	
	Our strategy is to apply the induction argument by the number of rounds of interactions. Fix a pair of neighboring datasets $x, x'$. We consider two cases depending on whether the first message sent from the mechanism $\mathcal{M}$ or the adversary $B$. 
	
	
	\paragraph{Case 1.}  The adversary $B$ sends the first query $q_1$ to the mechanism $\mathcal{M}$. Fixing $q_1$, the subsequent interactive mechanism $\mathcal{M}_{q_1}$ with input $x$ is defined by
	$$\mathcal{M}_{q_1}(x, q_2, \ldots, q_m, r)=\mathcal{M}(x, q_1, \ldots, q_m, r).$$
	We claim that $\View ( A \leftrightarrow \mathcal{M}_{q_1} )$ consists of $m-1$ messages, and $\mathcal{M}_{q_1}$ satisfies $d$-$\mathcal{D}$ DP on the two neighboring datasets $x$ and $x'$. By induction, there exists a randomized interactive post-processing $\mathcal{P}_{q_1}$ and a pair of random variables $Y_{q_1}, Y'_{q_1}$ such that 
	$$D(Y_{q_1}, Y'_{q_1}) \preceq d,$$
	and 
	$$\mathcal{P}_{q_1}(Y_{q_1})\equiv \mathcal{M}_{q_1}(x) \quad \mathcal{P}_{q_1}(Y'_{q_1})\equiv \mathcal{M}_{q_1}(x').$$
	By coupling property, there exists a pair of random variables $Y$, $Y'$ and a randomized post-processing function $\mathcal{Q}_{q_1}$ such that $D(Y,Y')\preceq d$, and we have that
	$$\mathcal{Q}_{q_1}(Y)=Y_{q_1},$$
	$$\mathcal{Q}_{q_1}(Y')=Y'_{q_1}.$$
	So $Y$ and $Y'$ are produced by coupling all possible queries.
	Then the interactive post-processing $\mathcal{P}$ is defined by $\mathcal{P}_{q_1}\circ \mathcal{Q}_{q_1}$, i.e.,
	$$\mathcal{P}(y, q_1, q_2, \ldots, q_m)=\mathcal{P}_{q_1}(\mathcal{Q}_{q_1}(y), q_2, \ldots, q_m).$$


%\sv{I'd drop all the coins.  Also, it's confusing to use the prime $\mathcal{P}'$ for the second post-processing function, since we are using prime to represent what happens on the adjacent dataset $x'$.  Instead, I'd write $\mathcal{Q}_{q_1}$ for the second post-processing function.  And the proof is also missing the statement that $D(Y,Y')\preceq d$.}
	
	
	\paragraph{Case 2.} The mechanism $\mathcal{M}$ sends the first message $a_1$ to the adversary $B$. Let $q_1,\ldots q_{m-1}$ be the queries from the adversary, and $A_1,\ldots,A_m$ be messages from the mechanism. Fixing $A_1=a_1$, the subsequent interactive mechanism $\mathcal{M}_{a_1}$ is defined by 
	$$\mathcal{M}_{a_1}(x, q_1, \ldots, q_{m-1}; g_x(r))=\mathcal{M}(x, q_1, \ldots, q_{m-1}; r).$$
	
	$\mathcal{M}_{a_1}$ uses its randomness to choose uniformly from randomness of $\mathcal{M}$ conditioned on $\mathcal{M}(x)=a_1$. Specifically, let $g_x$ be a random transformation such that if $R$ is uniform random for $\mathcal{M}$, then for all $x$, $g_x(R)$ is uniform on the randomness of $\mathcal{M}$ conditioned on $\mathcal{M}(x)=a_1$.
	
	We define the subsequent adversary $B_{a_1}(A_2, \ldots, A_m)=B(a_1, A_2, \ldots, A_m)$.
	We know that for all adversary strategy $B\in \mathcal{B}$, we have $D(\View ( B \leftrightarrow \mathcal{M}(x) ), \View ( B \leftrightarrow \mathcal{M}(x') )) \preceq d$, so we have $$\sup_B D(\View ( B\leftrightarrow \mathcal{M}(x) ), \View ( B\leftrightarrow \mathcal{M}(x') ))\preceq d.$$ We have 
	\begin{align}
		&\sup_B D(\View( B\leftrightarrow \mathcal{M}(x) ), \View( B\leftrightarrow \mathcal{M}(x') )) \notag  \\
		=&\sup_B(\mathrm{ChainRule}_{A_1,A'_1}((D(\View(B_{a_1} \leftrightarrow \mathcal{M}_{a_1}(x)), \View(B_{a_1} \leftrightarrow \mathcal{M}_{a_1}(x')) ))_{a_1 \in \supp(A_1) \cap \supp(A'_1)}))  \label{eq.chainrule}  \\
		=&\sup_{ (B_{a_1})_{a_1 \in \supp(A_1) \cap \supp(A'_1)} } (\mathrm{ChainRule}_{A_1,A'_1}((D(\View(B_{a_1} \leftrightarrow \mathcal{M}_{a_1}(x)), \View(B_{a_1} \leftrightarrow \mathcal{M}_{a_1}(x')) ))_{a_1 \in \supp(A_1) \cap \supp(A'_1)})) \label{eq.productadv}\\
		=&\mathrm{ChainRule}_{A_1,A'_1}(\sup_B (D(\View(B_{a_1} \leftrightarrow \mathcal{M}_{a_1}(x)), \View(B_{a_1} \leftrightarrow \mathcal{M}_{a_1}(x'))) )_{a_1 \in \supp(A_1) \cap \supp(A'_1)} ), \label{eq.cont}
	\end{align}
	where \eqref{eq.chainrule} follows from the chain rule, and \eqref{eq.productadv} is because that in the case that the first message $a_1$ comes from the mechanism, specifying an adversary $B$ for the entire mechanism is equivalent to specifying $B_{a_1}$ for ever $a_1$, then the set of deterministic adversary strategies $B$ we need to sup over is a product set over adversary strategies $B_{a_1}$. Equation \eqref{eq.cont} follows from that the $\mathrm{ChainRule}_{A_1,A'_1}$ function is continuous with respect to each variable. 
	For every $a_1\in \supp(A_1) \cap \supp(A'_1)$, define $d_{a_1}=\sup_{B_{a_1}}D(\View(B_{a_1} \leftrightarrow \mathcal{M}_{a_1}(x)), \View(B_{a_1} \leftrightarrow \mathcal{M}_{a_1}(x')) )$.
	Then $\mathcal{M}_{a_1}$ is $d_{a_1}$-$\mathcal{D}$ DP, by induction, there exists a pair of random variables $Y_{a_1}, Y'_{a_1}$ and a post-processing $\mathcal{P}_{a_1}$ such that 
	$$D(Y_{a_1}, Y'_{a_1}) \preceq d_{a_1},$$
	and 
	$$\mathcal{P}_{a_1}(Y_{a_1})\equiv \mathcal{M}_{a_1}(x) \text{ and } \mathcal{P}_{a_1}(Y'_{a_1})\equiv \mathcal{M}_{a_1}(x').$$
	Let $Y_{A_1}$ be the random variable that defined as $Y_{A_1}|_{A_1=a_1}\sim Y_{a_1}$. $Y'_{A_1}$ is defined similarly.
    By the chain rule, we have 
	\begin{align*}
		\MoveEqLeft D((A_1,Y_{A_1}), (A'_1,Y'_{A_1})) \\
		&= \mathrm{ChainRule}_{A_1,A'_1}( (D(Y_{a_1}, Y'_{a_1}))_{a_1 \in \supp(A_1) \cap \supp(A'_1)}) \\
		&\preceq \mathrm{ChainRule}_{A_1,A'_1}( (d_{a_1})_{a_1 \in \supp(A_1) \cap \supp(A'_1)}) \tag{by monotonicity of $\mathrm{ChainRule}$} \\
		&=\mathrm{ChainRule}_{A_1,A'_1}( (\sup_{B_{a_1}}D(\View(B_{a_1} \leftrightarrow \mathcal{M}_{a_1}(x)), \View(B_{a_1} \leftrightarrow \mathcal{M}_{a_1}(x')) ))_{a_1 \in \supp(A_1) \cap \supp(A'_1)} )\\
		&=\mathrm{ChainRule}_{A_1,A'_1}(\sup_B (D(\View(B_{a_1} \leftrightarrow \mathcal{M}_{a_1}(x)), \View(B_{a_1} \leftrightarrow \mathcal{M}_{a_1}(x'))) )_{a_1 \in \supp(A_1) \cap \supp(A'_1)} )\\
		&=\sup_{ B} (\mathrm{ChainRule}_{A_1,A'_1}((D(\View(B_{a_1} \leftrightarrow \mathcal{M}_{a_1}(x)), \View(B_{a_1} \leftrightarrow \mathcal{M}_{a_1}(x')) ))_{a_1 \in \supp(A_1) \cap \supp(A'_1)}))\\
		&\preceq d
	\end{align*}
	Let $Y=(A_1,Y_{A_1})$ and $Y'=(A'_1,Y'_{A_1})$, we define the post-processing $\mathcal{P}$ as 
	$$\mathcal{P}((a_1,y), q_1, \ldots, q_{m-1})=(a_1, \mathcal{P}_{a_1}(y,  q_1, \ldots, q_{m-1})).$$
	
	
	
\end{proof}

We now use Theorem \ref{thm.post_gen} to prove that
the concurrent composition of interactive mechanisms can be reduced to the composition of the non-interactive mechanisms. 
%As a result, any composition theorems for non-interactive $d$-$\mathcal{D}$ DP mechanisms extend to the concurrent composition of interactive $d$-$\mathcal{D}$ DP mechanisms. We now provide the proof of Theorem \ref{thm.concomp_d}.

\begin{theorem}[Theorem \ref{thm.fdp} generalized]\label{thm.concomp_d}
	Suppose that the generalized probability distance $(\mathcal{D}, \preceq, D)$ satisfies the chain rule, every $d\in \mathcal{D}$ satisfies the coupling property, and $(\mathcal{D}, \preceq)$ is complete. Suppose for all non-interactive mechanism $\mathcal{M}_1, \ldots, \mathcal{M}_k$ such that $\mathcal{M}_i$ is $d_i$-$\mathcal{D}$ DP for $i=1,2 \ldots, k$, their composition $\comp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ is $d$-$\mathcal{D}$ DP, then the concurrent composition $\concomp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$  of interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ such that $\mathcal{M}_i$ is $d_i$-$\mathcal{D}$ DP is also $d$-$\mathcal{D}$ DP.
\end{theorem}



\begin{proof}[Proof of Theorem \ref{thm.concomp_d}]
	
	
	
	Following Theorem \ref{thm.post_gen}, for every interactive $d_j$-$\mathcal{D}$ DP mechanism $\mathcal{M}_j$, $j=1,\ldots, k$, and every pair of neighboring datasets $x,x'$, there exists a pair of of random variables $Y_j,Y'_j$ and an interactive post-processing $\mathcal{P}_j$ such that $D(Y_j, Y'_j)\preceq d_j$, and for every adversary $B\in \mathcal{B}$, $\View(B\leftrightarrow \mathcal{M}_j(x))$ (resp.,$\View(B\leftrightarrow \mathcal{M}_j(x'))$ ) is identically distributed as $\View(B\leftrightarrow \mathcal{P}_j(Y_j))$ (resp., $\View(B\leftrightarrow \mathcal{P}_j(Y'_j))$). Since $Y_j,Y'_j$, $j=1,\ldots, k$, are noninteractive random variables, which can be viewed as the output distributions of a noninteractive mechanism $\mathcal{N}_j$ on $x,x'$. Suppose $\comp(\mathcal{N}_1, \ldots, \mathcal{N}_k)$ is $d$-$\mathcal{D}$ DP. By the post-processing property, we know that $\comp((\mathcal{P}_1(\mathcal{N}_1), \ldots,\mathcal{P}_k(\mathcal{N}_k))$ is also $d$-$\mathcal{D}$ DP. Therefore, we have that $\concomp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ is also $d$-$\mathcal{D}$ DP.
	
\end{proof}


%\begin{corollary}[Concurrent Composition]\label{thm.concomp}
%	If the generalized distance $\mathcal{D}$ satisfies the chain rule, and for any $d\in \mathcal{D}$ satisfies the coupling property, then suppose that for all non-interactive mechanism $\mathcal{M}_1, \ldots, \mathcal{M}_k$ such that $\mathcal{M}_i$ is $d_i$-$\mathcal{D}$ DP for $i=1,2 \ldots, k$, their composition $\comp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ is $d$-$\mathcal{D}$ DP, then the concurrent composition $\concomp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ of interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ is also $d$- $\mathcal{D}$ DP.
%\end{corollary}

%\section{Characterization of $f$-DP}
%
%In this section, we show that $f$-DP is an example of the generalization DP that satisfies the three basic properties. 
%We also prove that $f$-DP also satisfies the coupling property and the chain rule, and therefore, Theorem \ref{thm.post_gen} and Corollary \ref{thm.concomp} hold for $f$-DP. 
%
%$(\eps, \delta)$-DP is equivalent to $f_{\eps,\delta}$-DP, where $f_{\eps,\delta}=\max\{0, 1-\delta-\exp(\eps)\alpha, \exp(-\eps)(1-\delta-\alpha)\}$ \cite{wasserman2010statistical, dong2019gaussian}. Thus, the optimal composition theorem extends to approximate DP interactive mechanisms. This was raised as an open problem by \cite{vadhan2021concurrent}.


%\begin{lemma}
%	$f$-DP satisfies $d$-$\mathcal{D}$ DP. The partially ordered set $\mathcal{D}$ is defined as $(\mathcal{F}, \preceq)$, where $\mathcal{F}$ is a set of trade-off functions. The partially ordering is defined as $d_1\preceq d_2$ if  $d_1(\alpha)\ge d_2(\alpha)$ holds  for all $\alpha \in [0,1]$, and the distance mapping is the trade-off function in Definition \ref{def.fdp}.
%	%has the joint convexity and completeness
%\end{lemma}

%\begin{proof}
%	We will show that $f$-DP satisfies the three properties.
%	First, $f$-DP is preserved under post-processing. 
%	We now show the joint convexity of $f$-DP. Define $D(X_i, X'_i)\le d$ if the tradeoff function satisfies $T(X_i, X'_i)\ge f_d$. For any random variable $I$, suppose it takes value $i\in \mathcal{I}$ with probability $p_i$, where $\sum_i p_i=1$.  We have
%	\begin{align}
	%		T(X_I, X'_I)(\alpha)&=\inf_{\phi}\{ E_{X'_I}[1-\phi]: E_{X_I}[\phi]\le \alpha   \}  \notag \\
	%		&=\inf_{\phi}\{ E_{i\sim I}E_{X'_i} [1-\phi]: E_{i\sim I}E_{X_i}[\phi]\le \alpha  \} \notag  \\
	%		&=\inf_{\phi}\{ \sum_{i\in \mathcal{I}}p_i  E_{X'_i} [1-\phi]:   \sum_{i\in \mathcal{I}}p_iE_{X_i}[\phi]\le \alpha      \} \notag  \\
	%		&=\inf_{\alpha_i}\{ \sum_{i\in \mathcal{I}}p_i f_d(\alpha_i): \sum_{i\in \mathcal{I}}p_i \alpha_i \le \alpha \} \notag \\
	%		&\ge \inf_{\alpha_i}\{ f_d(\sum_{i\in \mathcal{I}} p_i\alpha_i) :  \sum_{i\in \mathcal{I}}p_i \alpha_i \le \alpha  \} \label{eq.joint} \\
	%		&= f_d(\alpha), \notag
	%	\end{align}
%	where inequality \eqref{eq.joint} follows from the convexity property of $f$. Therefore, we have $D(X_I, X'_I)\le d$. We complete the proof of the joint convexity of $f$-DP. 
%	
%	Then we show the completeness of $f$-DP. 	Since the distance for any pairs of random variables is defined by tradeoff functions, we shall show that $\sup_{f\in \mathcal{F}} f$ exists to prove the completeness property. For finite set, it suffices to show the supremum of two elements exists.  We define $h\succeq f$ if for all $\alpha\in[0,1]$, $h(\alpha)\le f(\alpha)$ holds.  For two tradeoff functions $f$ and $g$, let $h:=\sup(f, g)$ denotes the supremum. Then we have 
%	\begin{equation*}
	%		h(\alpha)=\inf_{p,\alpha_1,\alpha_2}\{ pf(\alpha_1)+(1-p)g(\alpha_2): p\alpha_1+(1-p)\alpha_2=\alpha  \}.
	%	\end{equation*}
%	We shall show that for any tradeoff function $h'$ such that $h' \succeq f$ and $h' \succeq g$, then $h' \succeq h$. For any $\alpha \in [0,1]$, if $h'(\alpha)\le f(\alpha)$ and $h'(\alpha)\le g(\alpha)$. By the convexity of $h'$,  $h'(\alpha)\le ph'(\alpha_1)+(1-p)h'(\alpha_2)$ holds for any $p\in [0,1]$ and any $\alpha_1$ and $\alpha_2$ such that $p\alpha_1+(1-p)\alpha_2\le \alpha$. Then we have $h'(\alpha)\le pf(\alpha_1)+(1-p)g(\alpha_2)$. Thus, we have  $h'(\alpha)\le \inf_{p,\alpha_1,\alpha_2}\{ pf(\alpha_1)+(1-p)g(\alpha_2): p\alpha_1+(1-p)\alpha_2=\alpha  \} = h(\alpha)$, and $h' \succeq h$.
%\end{proof}


%\begin{theorem}[Coupling Property of $f$-DP]
%	Suppose we have random variables $X_0$, $X_1$  and $X'_0$, $X'_1$ such that 
%	\begin{equation*}
	%		T(X_0,X'_0) \ge f \quad \text{and} \quad T(X_1,X'_1)\ge f,
	%	\end{equation*}
%	for any trade-off function $f$.
%	Then there exists random variables $Y=(Y_0, Y_1)$ and $Y'=(Y'_0, Y'_1)$, such that  $Y_q \equiv X_q$ and $Y'_q \equiv X'_q$   hold for any $q\in\{0,1\}$, and we have
%	\begin{equation*}
	%		T((Y_0,Y_1)||(Y'_0,Y'_1))\ge f.
	%	\end{equation*}
%\end{theorem}
%
%\begin{proof}
%	
%	Let $P, P'$ be a pair of random variables that satisfies $T(P, P')=f$. 
%	By the Blackwell theorem (Theorem 2.10 in \cite{dong2019gaussian} , also see Theorem 2.5 in \cite{kairouz2015composition}), since $T(P, P')=f\le T(X_0, X'_0)$, there exists a randomized algorithm $Proc_1$ such that $Proc_1(P), Proc_1(P')$ is identically distributed to $X, X'$, respectively. Similarly, since $T(P, P')=f\le T(X_1, X'_1)$, there exists a randomized algorithm $Proc_2$ such that $Proc_2(P), Proc_2(P')$ is identically distributed to $X_1, X'_1$, respectively. We denote a coupling of $X_0$ and $X'_0$ as $(Y_0, Y'_0)$, where $Y_0$ and $Y'_0$ have the same distribution as $X_0$ and $X'_0$, respectively. We also denote a coupling of $X_1$ and $X'_1$ as $(Y_1, Y'_1)$. Then the trade-off function between the two couplings satisfies the following inequality.
%	\begin{align}
	%		T((Y_0,Y_1),(Y'_0,Y'_1))&=T((Proc_1(P), Proc_2(P)), (Proc_1(P'), Proc_2(P')))  \notag \\
	%		&\ge T(P,P') \label{eq2} \\
	%		&=f,
	%	\end{align}
%	where Equation \eqref{eq2} follows from Lemma 2.9 in \cite{dong2019gaussian}.
%\end{proof}
%
%
%\begin{theorem}[Chain Rule of $f$-DP]
%	The class of $f$-DP where $\mathcal{D}$ is defined as $\{f \text{ is a trade-off function}\}$ satisfies the chain rule property. The Chains Rule function is given as 
%	\begin{equation*}
	%		ChainRule_{X,X'}((f_x)_{x\in support(X)\cap support(X') })=\inf_{\alpha_x\in[0,1]}\{ E_{x\in X'}[f_x(\alpha_x)]: E_{x\in X}[\alpha_x]\le \alpha  \}.
	%	\end{equation*}
%\end{theorem}
%
%\begin{proof}
%	
%	Let $X$ and $X'$ denote the output of a mechanism $\mathcal{M}_0$ on two fixed neighboring databases $x$ and $x'$, respectively, and let $Y$ and $Y'$ denote the output of a mechanism $\mathcal{M}_1$ on $D_0$ and $D_1$, respectively. For a given instance $x_0 \in support(X)\cap support(X')$, we define 
%	\begin{equation}\label{def.fx0}
	%		f_{x_0}=T(Y|_{X=x_0}, Y'|_{X'=x_0})=\inf\{\beta_\phi(X'=x_0): \alpha_\phi(X=x_0) \le \alpha\}. 
	%	\end{equation}
%	The type I and type II error of any decision rule $\phi$ given the event that $\{X=X'=x_0\}$ are given as follows.
%	\begin{equation*}
	%		\alpha_\phi=E_{(X, Y)}[\phi]=E_{X}[E_{Y}[\phi|X=x_0]]=E_{X}[\alpha_\phi(X=x_0)],
	%	\end{equation*}
%	and 
%	\begin{equation*}
	%		\beta_\phi=E_{(X', Y')}[\phi]=E_{X'}[E_{Y'}[\phi|X'=x_0]]=E_{X'}[\beta_\phi(X'=x_0)].
	%	\end{equation*}	
%	For any fixed $x_0 \in support(X)\cap support(X')$ and any decision rule $\phi$, by the definition of $f_{x_0}$, we have 
%	\begin{equation*}
	%		\beta_\phi(X'=x_0)\ge f_{x_0}(\alpha_\phi(X=x_0)).
	%	\end{equation*}
%	Therefore, the trade-off function between $(X,Y)$ and $(X',Y')$ satisfies the following inequality:
%	\begin{align}
	%		T((X,Y),(X',Y'))(\alpha)=\inf\{ \beta_\phi:\alpha_\phi\le \alpha  \} &= \inf\{ E_{X'}[\beta_\phi(X'=x_0)]: E_{X'}[\alpha_\phi(X'=x_0)]\le \alpha \} \notag \\ 
	%		&\ge \inf \{E_{X'}[f_{x_0}(\alpha_\phi(X=x_0))]: E_{X}[\alpha_\phi(X=x_0)]\le \alpha \}. \label{eq.5}
	%	\end{align}
%	One the other hand, by the definition of $f_{x_0}$, for any $0<\alpha_{x_0}<1$ and $\delta>0$, there exists a decision rule $\phi_\delta$ such that $\beta_{\phi_\delta}(X'=x_0)\le f_{x_0}(\alpha_{x_0})+\delta$, and $\alpha_{\phi_\delta}\le \alpha_{x_0}$. Then we have
%	\begin{equation*}
	%		\inf \{E_{X'}[f_{x_0}(\alpha_{x_0})]: E_{X}[\alpha_{x_0}]\le \alpha \}\ge \inf \{E_{X'}[\beta_{\phi_\delta}(X'=x_0)-\delta]: E_{X}[\alpha_{x_0}]\le \alpha \}. 
	%	\end{equation*}
%	Let $\delta$ go to $0$, the decision function $\phi_\delta$ will converge to the decision rule $\phi*$ such that the infimum is reached, and thus, we arrive at 
%	\begin{align}\label{eq.6}
	%		\inf \{E_{X'}[f_{x_0}(\alpha_{x_0})]: E_{X}[\alpha_{x_0}]\le \alpha \} &\ge \inf \{E_{X'}[\beta_{\phi*}(X'=x_0)]: E_{X}[\alpha_{x_0}]\le \alpha \} \notag \\
	%		&\ge T(X, Y)(\alpha)T((X,Y),(X',Y'))(\alpha). 
	%	\end{align}
%	Combining Equation \eqref{eq.5} and  Equation \eqref{eq.6}. we have
%	\begin{equation}\label{eq.7}
	%		T((X,Y),(X',Y'))(\alpha)=\inf \{E_{X'}[f_{x_0}(\alpha_{x_0})]: E_{X}[\alpha_{x_0}]\le \alpha \}.
	%	\end{equation}
%	
%	Next, we shall show that the ChainRule function $f$ defined in \eqref{eq.f_chain} is continuous. 
%	\begin{equation}\label{eq.f_chain}
	%		f=ChainRule_{X,X'}((f_x)_{x\in support(X)\cap support(X') })=\inf_{\alpha_x\in[0,1]}\{ E_{x\in X'}[f_x(\alpha_x)]: E_{x\in X}[\alpha_x]\le \alpha  \}
	%	\end{equation}
%	
%	Suppose $support(X)\cap support(X')$ has finite elements, and we have $X= x_j$ with probability $p_j$ and $X'=x_j$ with probability $p'_j$. Then we can write the ChainRule function as 
%	\begin{equation*}
	%		ChainRule_{X,X'}((f_x)_{x\in support(X)\cap support(X') }) = \inf_{\alpha_x\in[0,1]}\{ \sum_j p'_j f_{x_j}(\alpha_{x_j}): \sum_j p_j \alpha_{x_j}\le \alpha  \}
	%	\end{equation*}
%	
%	We hope to show that $f(\sup(S))=\sup(f(S))$ for every set $S$. Without loss of generality, we consider the set $S=\{ (f_{x_j})_{x_j \in support(X)\cap support(X') }, (g_{x_j})_{x_j \in support(X)\cap support(X') }  \}$.  Let 
%	\begin{equation*}
	%		f(\alpha)=ChainRule((f_{x_j})_{x_j})=\inf_{\alpha_{x_j}} \{ \sum_j p'_jf_{x_j}(\alpha_{x_j}):\sum_jp_j \alpha_{x_j}\le \alpha \},
	%	\end{equation*}
%	and 
%	\begin{equation*}
	%		g(\alpha)=ChainRule((g_{x_j})_{x_j})=\inf_{\alpha_{x_j}}  \{ \sum_j p'_jg_{x_j}(\alpha_{x_j}):\sum_jp_j \alpha_{x_j}\le \alpha \},
	%	\end{equation*}
%	We consider the $sup(f, g)$
%	Let $h$ denote $sup(f, g)$, 
%	\begin{align*}
	%		h(\alpha)&=\sup(f(\alpha), g(\alpha))=\inf_{p,\alpha_1, \alpha_2}\{ pf(\alpha_1)+(1-p)g(\alpha_2 ) : p\alpha_1+(1-p)\alpha_2=\alpha  \}\\
	%		&=\inf_{p,\alpha_1, \alpha_2}\{ p \inf\{ \sum_jp'_jf_{x_j}(\alpha_{x_j}): \sum_j p_j \alpha_{x_j}\le \alpha_1\} + (1-p)\inf\{  \sum_jp'_jg_{x_j}(\alpha'_{x_j}): \sum_j p_j \alpha'_{x_j}\le \alpha_2\} \\ 
	%		& : p\alpha_1+(1-p)\alpha_2 = \alpha     \}
	%	\end{align*}
%	
%	On the other hand, 
%	\begin{align*}
	%		ChainRule_{X,X'}(\sup(S))&=\inf_{\alpha_x\in [0,1]}\{ \sum_j p'_j h_{x_j}(\alpha_{x_j}): \sum_j p_j \alpha_{x_j}\le \alpha     \} \\
	%		&=\inf_{\alpha_x\in [0,1]} \{ \sum_j p'_j  \inf_{p, \alpha_{x_j}, \alpha'_{x_j}}\{ pf_{x_j}(\alpha_{x_j})+(1-p)g_{x_j}(\alpha'_{x_j}): p\alpha_{x_j}+(1-p)\alpha'_{x_j}=\alpha_j\}: \sum_j p_j\alpha_{x_j}\le \alpha  \}. \\
	%		&=\inf_{ \substack{\sum_jp_j\alpha_{x_j}=\alpha_1\\ \sum_jp_j\alpha'_{x_j}=\alpha_2 \\ p\alpha_1+(1-p)\alpha_2=\alpha } }\{p \sum_j p_j f_{x_j}(\alpha_{x_j}) + (1-p) \sum_j p_j g_{x_j}(\alpha'_j) \}
	%	\end{align*}
%	
%	Therefore, $ChainRule_{X,X'}(\sup(S))=\sup(ChainRule_{X,X'}(S))$.
%	
%	
%	%$\inf_{\alpha_{x_j}}\{ \sum_j p'_j \sup(f_{x_j}, g_{x_j}) : \sum_jp_j \alpha_{x_j}\le \alpha   \}$
%	
%	%\todo{change the following paragraph to distance.}
%	%Now we verify the two conditions in Definition \ref{def.chain}. For any $f$-DP where $f>0$ and $x_0\in support(X)\cap support(X')$, $T(Y|_{X=x_0}, Y'|_{X'=x_0})\ge f_{x_0}$, there exists a $f_{x_0}$-DP relation such that $X_1|_{X_0=x_0}$ and  $Y_1|_{Y_0=x_0}$ satify $f_{x_0}$-DP relation. For any random variable $(X_0,X_1')$ and $(Y_0,Y_1')$ such that $f_{x_0}$-DP relation for any instance $x_0$, then following Equation \eqref{eq.7}, $(X_0,X_1')$ and $(Y_0,Y_1')$ satisfy $f$-DP relation, completing the proof.
%	
%\end{proof}
%
%
%\begin{corollary}
%	For any interactive $f$-DP mechanism $\mathcal{M}$, and any pair of neighboring dataset $x,x'$, there exists a non-interactive $f$-DP mechanism $\mathcal{N}$ and an interactive post-processing mechanism $T$ such that for every adversary $A \in \mathcal{A}$, we have 
%	\begin{align}
	%		View(\mathcal{A}, \mathcal{M}(x))\equiv View(A, T(N(x)))
	%		&&
	%		View(\mathcal{A}, \mathcal{M}(x'))\equiv View(A, T(N(x'))).
	%	\end{align}
%\end{corollary}
%
%\begin{corollary}
%	Suppose that for all non-interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ such that $\mathcal{M}_i$ is $f_i$-DP for $i=1,2 \ldots, k$, their composition $\comp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ is $f$-DP, then the concurrent composition $\concomp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ of interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ is also $f$-differentially private.
%\end{corollary}
%
%
%

\section{Concurrent Composition of R\'enyi DP}\label{sec.RDP}

In this section, we give a different and simpler proof of the optimal concurrent composition of R\'enyi DP given in \cite{lyu2022composition}:

\begin{theorem}[\cite{lyu2022composition}]\label{thm.rdp2}
	For all $\alpha>1$, $k\in \mathbb{N}$, $\eps_1,\ldots, \eps_k>0$, and all interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ such that $\mathcal{M}_i$ is $(\alpha,\eps_i)$-RDP for $i=1,2 \ldots, k$, 
	the concurrent composition $\concomp(\mathcal{M}_1, \ldots, \mathcal{M}_k)$ of interactive mechanisms $\mathcal{M}_1, \ldots, \mathcal{M}_k$ is $(\alpha,\sum_{i=1}^k\eps_i)$-RDP.
\end{theorem}

We prove this theorem by characterizing optimal $\alpha$-RDP adversary strategy in Lemma \ref{lemma.optadv}. 

\begin{definition}[Optimal $\alpha$-RDP adversary]
	For an interactive mechanism $\mathcal{M}$, and neighboring datasets $x$ and $x'$, an optimal $\alpha$-RDP adversary with respect to $x$ and $x'$ is a strategy $B^{\mathrm{OPT}}$ such that for all adversary strategies $B$, 
	\begin{equation*}
		D_\alpha( \View(B^{\mathrm{OPT}}\leftrightarrow \mathcal{M}(x)) || \View(B^{\mathrm{OPT}}\leftrightarrow \mathcal{M}(x'))   )\ge D_\alpha( \View(B\leftrightarrow \mathcal{M}(x)) || \View(B\leftrightarrow \mathcal{M}(x'))   ).
	\end{equation*}
\end{definition}


We show that the optimal adversary strategy against the concurrent composition of $k$ mechanisms can be decomposed as a product of optimal adversaries against each mechanism independently: 

\begin{lemma}\label{lemma.optconcomp}
	Let $B^{\mathrm{OPT} (1)}, B^{\mathrm{OPT} (2)}, \ldots, B^{\mathrm{OPT} (k)}$ be optimal $\alpha$-RDP adversaries against $\mathcal{M}_1, \mathcal{M}_2, \ldots, \mathcal{M}_k$. Then 
	\begin{equation*}
		B^{\mathrm{OPT}} =B^{\mathrm{OPT} (1)} \times B^{\mathrm{OPT} (2)} \times \ldots \times B^{\mathrm{OPT} (k)}
	\end{equation*}
is an optimal $\alpha$-RDP adversary against $\concomp(\mathcal{M}_1, \mathcal{M}_2, \ldots, \mathcal{M}_k)$, where $B^{\mathrm{OPT} (1)} \times B^{\mathrm{OPT} (2)}$ denotes the adversary's strategy where it takes $B^{\mathrm{OPT} (1)}$ to interact with $\mathcal{M}_1$ and takes $B^{\mathrm{OPT} (2)}$ to interact with $\mathcal{M}_2$.
\end{lemma}


%We show that the optimal adversary strategy against the concurrent composition of $k$ mechanisms can be decomposed as a product of optimal adversaries against each mechanism independently in Lemma \ref{lemma.optconcomp}. 
Although this property of the optimal adversary strategy can be derived as a consequence of the optimal concurrent composition of R\'enyi DP in \cite{lyu2022composition}, we take a different approach to first prove this property and then use it to prove the optimal concurrent composition theorem for R\'enyi DP. 

Our proof relies on the following two properties of R\'enyi divergence: the monotonicity property in Lemma \ref{lemma.monotone} and the independence property in Lemma \ref{lemma.indep}. The R\'enyi divergence is defined as follows.
\begin{definition}[R\'enyi divergence \cite{renyi1961measures}]
	For two probability distributions $P$ and $Q$, the R\'enyi divergence of order $\alpha>1$ is 
	\begin{equation*}
		D_\alpha(P||Q)=\frac{1}{\alpha-1}\log \mathrm{E}_{x\sim Q} \left[\frac{P(x)}{Q(x)}\right]^\alpha.
	\end{equation*}
\end{definition}

\begin{lemma}\label{lemma.monotone}
	For any two tuples of jointly distributed random variables $(U,V,W)$ and $(U',V',W')$ over the same measureable space,  if for every $u\in \supp(U)$, we have 
	\begin{equation*}
		D_\alpha(V|_{U=u}||V'|_{U'=u}) \le D_\alpha(W|_{U=u}||W'|_{U'=u}),
	\end{equation*}
then 
	\begin{equation*}
	D_\alpha((U, V)||(U',V')) \le D_\alpha((U,W)||(U',W')).
\end{equation*}
\end{lemma}

\begin{proof}
	\begin{align*}
	\MoveEqLeft D_\alpha((U, V)||(U',V')) \\
	&=\frac{1}{\alpha-1}\log \sum_{u,v}\frac{ \left( \Pr(U=u)\Pr(V=v|U=u) \right)^\alpha }{ \left( Pr(U'=u)\Pr(V'=v|U'=u) \right)^{\alpha -1} } \\
	&=\frac{1}{\alpha-1}\log \sum_{u}\frac{ \left( \Pr(U=u) \right)^\alpha} { \left( Pr(U'=u)\right)^{\alpha -1} }\left( \sum_{v}\frac{ \left( \Pr(V=v|U=u) \right)^\alpha} { \left( Pr(V'=v|U'=u)\right)^{\alpha -1} }\right) \\
	&=\frac{1}{\alpha-1}\log \sum_{u}\frac{ \left( \Pr(U=u) \right)^\alpha} { \left( Pr(U'=u)\right)^{\alpha -1} }\left( \exp(\alpha-1) D_\alpha(V|_{U=u}||V'|_{U'=u}) \right).
	\end{align*}
Hence, $D_\alpha((U, V)||(U',V')) $ is monotonically increasing if $D_\alpha(V|_{U=u}||V'|_{U'=u})$ increases. So if $D_\alpha(V|_{U=u}||V'|_{U'=u}) \le D_\alpha(W|_{U=u}||W'|_{U'=u})$, then we have $D_\alpha((U, V)||(U',V')) \le D_\alpha((U,W)||(U',W')).$

\end{proof}

\begin{lemma}\label{lemma.indep}
	For any two pairs of random variables $U, U'$ and $V, V'$, if $U$ and $V$ ($U'$ and $V'$ resp.) are independent, then 
	\begin{equation*}
		D_\alpha((U, V)||(U',V')) =D_\alpha(U||U') + D_\alpha(V||V').
	\end{equation*}
\end{lemma}

\begin{proof}
	\begin{align*}
	\MoveEqLeft	D_\alpha((U, V)||(U',V')) \\
	&=\frac{1}{\alpha-1}\log \sum_{u,v}\frac{ \left( \Pr(U=u)\Pr(V=v) \right)^\alpha }{ \left( Pr(U'=u)\Pr(V'=v) \right)^{\alpha -1} } \\
	&=\frac{1}{\alpha-1}\log \sum_{u}\frac{ \left( \Pr(U=u) \right)^\alpha} { \left( Pr(U'=u)\right)^{\alpha -1} }\left( \exp(\alpha-1) D_\alpha(V||V') \right) \\
	&=D_\alpha(U||U') + D_\alpha(V||V').
	\end{align*}
\end{proof}


The following lemma describes the optimal adversary's strategy against an interactive mechanism. 
 The proof of Lemma \ref{lemma.optadv} uses the monotonicity property of R\'enyi divergence.

\begin{lemma}\label{lemma.optadv}
	The optimal adversary $B^{\mathrm{OPT}}$ with respect to $x$ and $x'$ , which is the adversary strategy that maximizes the R\'enyi divergence of the views for all fixed $x,x'$,
	chooses the first query $q_1$ to maximize 
\begin{equation*}
D_\alpha\left(  \left(A_1, \View\left(   B^{\mathrm{OPT}}_{q_1, A_1} \leftrightarrow M_{q_1, A_1}(x)  \right)  \right)  ||  \left(A'_1, \View \left(  B^{\mathrm{OPT}}_{q_1, A'_1} \leftrightarrow M_{q_1, A'_1}(x')  \right)  \right)    \right) ,
\end{equation*}
where $A_1= \mathcal{M}(x,q_1)$ and $A'_1= \mathcal{M}(x',q_1)$, and $B^{\mathrm{OPT}}_{q_1, a_1}$ is any optimal adversary against $\mathcal{M}_{q_1, a_1}$, which denotes the subsequent mechanism when fixing $q_1, a_1$.
\end{lemma}

\begin{proof}
We decompose the view of the adversary into two parts: the first answer $A_1$ to the query $q_1$, and the view of the subsequent interaction. Fixing $q_1$, for every adversary $B$, we have
\begin{align}
	\MoveEqLeft D_\alpha( \View(B\leftrightarrow \mathcal{M}(x)) || \View(B\leftrightarrow \mathcal{M}(x'))   ) \label{eq.divergence} \\
&=D_\alpha\left(  \left(A_1(q_1), \View\left(   B_{q_1, A_1} \leftrightarrow \mathcal{M}_{q_1, A_1}(x)  \right)  \right)  ||  \left(A'_1(q_1), \View \left(  B_{q_1, A'_1} \leftrightarrow \mathcal{M}_{q_1, A'_1}(x')  \right)  \right)    \right) , \notag
\end{align}
where $B_{q_1, A_1} \leftrightarrow \mathcal{M}_{q_1, A_1}$ denotes the subsequent interaction. For every $a_1\in \supp(A_1)\cap\supp(A'_1)$ and for every $B_{q_1, A_1}$, by the definition of $B^{\mathrm{OPT}}_{q_1, A_1}$, we have 
\begin{align*}
	\MoveEqLeft   D_\alpha\left(  \View(B_{q_1, A_1}\leftrightarrow \mathcal{M}_{q_1,A_1}(x))|_{A_1=a_1} || \View(B_{q_1,A'_1}\leftrightarrow \mathcal{M}_{q_1,A'_1}(x'))|_{A'_1=a_1}   \right)  \\
	&\le D_\alpha \left( \View(B^{\mathrm{OPT}}_{q_1, A_1}\leftrightarrow \mathcal{M}_{q_1,A_1}(x))|_{A_1=a_1} || \View(B^{\mathrm{OPT}}_{q_1,A'_1}\leftrightarrow \mathcal{M}_{q_1,A'_1}(x'))|_{A'_1=a_1}   \right).
\end{align*}
Thus, we have 
\begin{align}
	\MoveEqLeft  D_\alpha\left(  \left(A_1(q_1), \View\left(   B_{q_1, A_1} \leftrightarrow \mathcal{M}_{q_1, A_1}(x)  \right)  \right)  ||  \left(A'_1(q_1), \View \left(  B_{q_1, A'_1} \leftrightarrow \mathcal{M}_{q_1, A'_1}(x')  \right)  \right)    \right) \notag \\
&\le D_\alpha\left(  \left(A_1(q_1), \View\left(   B^{\mathrm{OPT}}_{q_1, A_1} \leftrightarrow \mathcal{M}_{q_1, A_1}(x)  \right)  \right)  ||  \left(A'_1(q_1), \View \left(  B^{\mathrm{OPT}}_{q_1, A'_1} \leftrightarrow \mathcal{M}_{q_1, A'_1}(x')  \right)  \right)    \right), \label{eq.optB}
\end{align}
where \eqref{eq.optB} follows from Lemma \ref{lemma.monotone}. It implies that in order to maxmize \eqref{eq.divergence}, it suffices to choose $q_1$ to maximize the quantity in \eqref{eq.optB}.
\end{proof}


We then use Lemma \ref{lemma.optadv} to prove Lemma \ref{lemma.optconcomp}.

%characterize the optimal adversary strategy against the concurrent composition of $k$ mechanisms $\concomp (M_1, M_2, \ldots, M_k)$ in Lemma \ref{lemma.optconcomp}.


\begin{proof}[proof of Lemma \ref{lemma.optconcomp}.]
	We will use induction on the rounds of messages to prove this lemma. We can use induction argument because of the assumption of finite communication. Without loss of generality, suppose the first query from the adversary is sent to $\mathcal{M}_1$, and we use $\concomp = \concomp(\mathcal{M}_1, \mathcal{M}_2, \ldots, \mathcal{M}_k)$ to simplify the notation.
	Following Lemma \ref{lemma.optadv}, the optimal adversary $B^{\mathrm{OPT}}$ chooses $q_1$ as follows.
	\begin{equation*}
	B^{\mathrm{OPT}}=\argmax_{q_1}  D_\alpha\left(  \left(A_1, \View\left(   B^{\mathrm{OPT}}_{q_1, A_1} \leftrightarrow \concomp_{q_1, A_1}(x)  \right)  \right)  ||  \left(A'_1, \View \left(  B^{\mathrm{OPT}}_{q_1, A'_1} \leftrightarrow \concomp_{q_1, A'_1}(x')  \right)  \right)    \right),
	\end{equation*}
where $A_1=\mathcal{M}_1(x,q_1)$ and $A'_1=\mathcal{M}_1(x',q_1)$.
By induction, we assume that $B^{\mathrm{OPT}}_{q_1, A_1}= B^{\mathrm{OPT} (1)}_{q_1, A_1} \times  B^{\mathrm{OPT} (2)} \times \ldots \times B^{\mathrm{OPT} (k)} $. Let $V_{q_1, A_1}=\View\left( B^{\mathrm{OPT} (1)}_{q_1, A_1} \leftrightarrow \mathcal{M}_{q_1, A_1}(x)  \right) $, and similarly, $V'_{q_1, A_1}=\View\left( B^{\mathrm{OPT} (1)}_{q_1, A'_1} \leftrightarrow \mathcal{M}_{q_1, A'_1}(x')  \right) $. Let $\tilde{V}=\View \left(  B^{\mathrm{OPT} (2)} \times \ldots \times B^{\mathrm{OPT} (k)} \leftrightarrow \concomp(\mathcal{M}_2, \ldots, \mathcal{M}_k) (x) \right) $ and \\ $\tilde{V}'=\View \left(  B^{\mathrm{OPT} (2)} \times \ldots \times B^{\mathrm{OPT} (k)} \leftrightarrow \concomp(\mathcal{M}_2, \ldots, \mathcal{M}_k)(x') \right) $. With these notations, we have
\begin{align}
	\MoveEqLeft \argmax_{q_1}  D_\alpha\left(  \left(A_1, \View\left(   B^{\mathrm{OPT}}_{q_1, A_1} \leftrightarrow \concomp_{q_1, A_1}(x)  \right)  \right)  ||  \left(A'_1, \View \left(  B^{\mathrm{OPT}}_{q_1, A'_1} \leftrightarrow \concomp_{q_1, A'_1}(x')  \right)  \right)    \right) \notag \\
	=& \argmax_{q_1} D_\alpha\left(  \left(  A_1, V_{q_1, A_1}, \tilde{V}  \right) || \left(  A'_1, V'_{q_1, A_1}, \tilde{V}'  \right)    \right) \notag  \\
	=& \argmax_{q_1} \left\lbrace  D_\alpha\left(  \left(  A_1, V_{q_1, A_1} \right) || \left(  A'_1, V'_{q_1, A_1} \right)    \right) + D_\alpha(\tilde{V}  ||  \tilde{V}' )  \right\rbrace , \tag{by Lemma \ref{lemma.indep}} \\
	=& \argmax_{q_1}  D_\alpha\left(  \left(  A_1, V_{q_1, A_1} \right) || \left(  A'_1, V'_{q_1, A_1} \right)    \right) \notag \\
	=&B^{\mathrm{OPT} (1)}.
\end{align}
Therefore, the optimal adversary $B^{\mathrm{OPT}}$ chooses $q_1$  just as the optimal adversary $B^{\mathrm{OPT}(1)}$ against only $M_1$. Since $B^{\mathrm{OPT}}_{q_1, A_1}= B^{\mathrm{OPT} (1)}_{q_1, A_1} \times  B^{\mathrm{OPT} (2)} \times \ldots \times B^{\mathrm{OPT} (k)} $, we have 
$B^{\mathrm{OPT}}=B^{\mathrm{OPT} (1)} \times  B^{\mathrm{OPT} (2)} \times \ldots \times B^{\mathrm{OPT} (k)} $, completing the proof.
\end{proof}


We now prove Theorem \ref{thm.rdp2} using Lemma \ref{lemma.optconcomp}.

\begin{proof}[Proof of Theorem \ref{thm.rdp2}]
Following Lemma \ref{lemma.optconcomp}, we have 
\begin{align*}
	\MoveEqLeft D_\alpha \left( \View \left( B^{\mathrm{OPT}} \leftrightarrow \concomp (x) \right)  ||  \View \left( B^{\mathrm{OPT}} \leftrightarrow \concomp (x') \right)   \right) \\
	=& D_\alpha \left( \View \left( B^{\mathrm{OPT}(1)} \leftrightarrow \mathcal{M}_1 (x) \right)  ||  \View \left( B^{\mathrm{OPT}(1)} \leftrightarrow \mathcal{M}_1(x') \right)   \right)+ \ldots \\
	&+ D_\alpha \left( \View \left( B^{\mathrm{OPT}(k)} \leftrightarrow \mathcal{M}_k (x) \right)  ||  \View \left( B^{\mathrm{OPT}(k)} \leftrightarrow \mathcal{M}_k(x') \right)   \right) \\
	=&\sum_i^k\eps_i,
\end{align*}
completing the proof.
\end{proof}





\section*{Acknowledgments}
We are grateful to Xin Lyu for pointing out the error in the proof of our previously claimed concurrent composition theorem for R\'enyi DP~\cite{lyu2022composition}. We also thank an anonymous reviewer for pointing out the error in our previous proof of continuity.





